Influential Recommender System

Traditional recommender systems are typically passive in that they try to adapt their recommendations to the user's historical interests. However, it is highly desirable for commercial applications, such as e-commerce, advertisement placement, and news portals, to be able to expand the users' interests so that they would accept items that they were not originally aware of or interested in to increase customer interactions. In this paper, we present Influential Recommender System (IRS), a new recommendation paradigm that aims to proactively lead a user to like a given objective item by progressively recommending to the user a sequence of carefully selected items (called an influence path). We propose the Influential Recommender Network (IRN), which is a Transformer-based sequential model to encode the items' sequential dependencies. Since different people react to external influences differently, we introduce the Personalized Impressionability Mask (PIM) to model how receptive a user is to external influence to generate the most effective influence path for the user. To evaluate IRN, we design several performance metrics to measure whether or not the influence path can smoothly expand the user interest to include the objective item while maintaining the user's satisfaction with the recommendation. Experimental results show that IRN significantly outperforms the baseline recommenders and demonstrates its capability of influencing users' interests.

==> Influential RS/conclusion.tex <==
We introduce a new recommendation paradigm termed \textit{Influential Recommender System} (\textit{IRS}), which proactively and incrementally expands a user's interest toward an objective item by recommending to the user a sequence of items. We design a Transformer-based sequential model \textit{Influential Recommender Network} (\textit{IRN}) with \textit{Personalized Impressionability Mask} (\textit{PIM}) to model, respectively, the sequential dependencies among the items and individual users' personalized acceptance of external influence. Evaluation metrics are carefully designed for the influential recommendation task. Experimental results show that \textit{IRN} significantly outperforms the baseline recommenders and demonstrate \textit{IRN}'s capability in smooth and progressive persuasion.

Since this is the first work that proposes the idea of influential recommendation, we are in the exploratory stage for this new recommendation problem. Many issues remain to be further studied.
We summarize the future work in the following directions.
(1) Extend the path-finding baseline by incorporating knowledge graphs (\textit{KG}). Knowledge graphs have been extensively used in recommendation systems, making them a natural fit of the \textit{IRS} framework. For example, we can model the user's historical interests as a subgraph and expand the subgraph toward the objective item.
(2) Improve the evaluation of unknown sequence-item interactions. Due to the limitation of the offline dataset used in this work, we utilize an evaluator to stimulate the user's interest in a new incoming item, which may incur bias in calculating the \textit{IRS} evaluation metrics. A better solution is to deploy the \textit{IRS} in an online recommendation platform where honest user feedback is available or to conduct a human experiment to evaluate the generated influence paths.
(3) Expand the scope of the objective in \textit{IRS}. In this work, the proposed framework aims at leading the user to like a single objective item, which naturally leads to a broader problem setting where the objective can be a collection of items, a category, a topic, etc. 
(4) Consider the stepwise dynamics in generating the influence path. For simplicity, we assume that the user passively accepts the recommended items and evaluates the influence path as a whole. However, in a more practical application scenario, it is important to consider the stepwise user response to a recommended item in approaching the objective. For example, a user may reject an intermediate item in a pre-scheduled influence path, and the \textit{IRS} needs to alter its strategy by recommending another item to persuade the user towards the objective.

% Consider shorten the conclusion

% (4) Integrate with content-based \textit{RS}. 

% (5) Comprehensive evaluation 

% Admittedly
% In future work, we will apply the proposed model to online datasets where feedback from real users is available. We also plan to consider more factors such as diversities and novelties in generating the influence path.
% (2) perform a more comprehensive evaluation on the persuasion path by considering other factors such as diversity, and (3) explore other potential methods (e.g. knowledge graph) to conduct progressive recommendation.

==> Influential RS/cover_letter.tex <==
\noindent\textbf{Dear Reviewers:}
% \section*{Response Letter}

\noindent We appreciate the time and effort that you dedicated to handling our paper, providing feedback and giving us the opportunity to submit a revised paper. We are grateful for the insightful comments and have incorporated suggestions made by the reviewers. All changes are highlighted within the manuscript in red color. The removed text and minor changes (e.g. corrected spelling and grammar mistakes) have not been highlighted. We hereby provide a point-by-point response below:

\begin{itemize}%[leftmargin=0.4cm]
    \item We have clarified a few confusing points raised by the reviewers, including the use of the testing dataset (as suggested by \textbf{Reviewer #4 O1}) at the end of Section IV-A, and replaced the term ``horizon" with ``interest" (as suggested by \textbf{Reviewer #7 O1}). 
    \item Following the suggestions by \textbf{Reviewer #5 O2}, we add comments in the experimental results (Section IV-D-6) regarding the scalability and robustness of the model.
    \item \textbf{Reviewer #7 O2\&O3} suggests comparing the proposed framework to traditional methods (e.g., minimum spanning tree, search algorithm, and shortest path algorithms).
    Following this suggestion, we replace one naive baseline solution \textit{Vec2Inf} with \textit{Pf2Inf} that adapts path-finding algorithms to the influential recommendation framework. We describe the new baseline framework in Section III-B. In the experiments, we added two new baseline approaches (i.e., Dijkstra and MST) under the \textit{Pf2Inf} framework. The experimental results are presented and discussed in Section IV-D. We also extended the future work regarding the traditional methods in Section V.
\end{itemize}
%Thanks again for all the time and patience of the anonymous reviewers. 
We will also publicly release the full code and scripts on GitHub upon acceptance (suggested by \textbf{Reviewer #5 O1}). 

==> Influential RS/experiment.tex <==
% \textcolor{red}{[ZHU: Experiment outlines are as follows: (1) Datasets, (2) Baselines, (3) Metrics, (4) experiment results, which include the overall comparison in terms of a few metrics, hyper-parameters analysis, and the visualization of generated recommendation path. I remove the content that discusses the user satisfaction results, since it is not the main focus of PRS and it seems difficult for the proposed framework to outperform the reported state-of-the-art method statistics. Notice that there are two ways to evaluate the results (with random target or existing target, which has corresponding metrics.)]}

We evaluate the proposed framework using two commonly used recommendation datasets. 
To meet the requirement of \textit{IRS}, we design several new metrics to assess the model performance.  
Since \textit{IRS} recommends an item sequence, many sequence-item interactions may not exist in the original dataset, making it difficult to evaluate the user's acceptance of these items.
To mitigate the problem, we use a trained \textit{evaluator} to provide probability measures for the unknown sequence-item interactions. 
We will explain in detail the experiment design and outcomes in the remaining sections.  

\begin{table}[tb]
    \centering
%     \setlength{\belowcaptionskip}{-5pt}
% 	\setlength{\abovecaptionskip}{3pt}
    \caption{Statistics of Datasets after Preprocessing. }
    \resizebox{0.45\textwidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
    \multirow{2}{*}{Dataset}&\multirow{2}{*}{Users}&\multirow{2}{*}{Items} &\multirow{2}{*}{Interactions}&\multirow{2}{*}{Density} &Avg. Items \\
    &&&&&per User\\
    \midrule
    % Movielens-100k&943&1,682&100,000&6.30\%&106.0\\
    Lastfm&896&2,682&28,220&1.17\%&31\\
    Movielens-1m&6,040&3,415&996,183&4.83\%&164\\
    % lastfm&992&107,296&19,150,868&?\%&\\
    \bottomrule
    % \multicolumn{6}{l}{\multirow{2}{*}{\small * Density here is calculated by $\frac{\mbox{Number of unique interactions}}{\mbox{Users}\times \mbox{Items}} $.}} \\
    \end{tabular}}
    \label{tab:datasets_info}
% 	\setlength{\belowcaptionskip}{-10pt}
% 	\setlength{\abovecaptionskip}{-2pt}
% 	\vspace{-5mm}
\end{table}

\subsection{Datasets}
Since online user-item interaction datasets with feedback from real users are not available, we design experiments based on offline datasets that are suitable for the influential recommendation. Specifically, we consider datasets that satisfy the following properties : (1) user-item interactions should exhibit sequential patterns and interaction timestamps are available, and (2) cost in user-item interactions should not be too high to be practical. 
% \textcolor{red}{it is not clear to me what is a decision cost, i.e., the cost (time taken) for the user to make a decision on whether to like or not like an item? or the cost of making a wrong decision?, etc.}
For example, e-commerce purchase datasets may not be suitable because promoting the objective item by asking the user to buy other items is less practical.  
Taking these requirements into consideration, we select two widely used datasets, namely, 
% Movielens-100k \footnote{https://grouplens.org/datasets/movielens/100k/} and 
Movielens-1m\footnote{https://grouplens.org/datasets/movielens/1m} and
Lastfm\footnote{https://grouplens.org/datasets/hetrec-2011/} which have timestamps indicating when the user-item interactions take place. 
Moreover, watching movies and listening to music have relatively low costs. 

% lastfm contains the listening habits for nearly one thousand users. The detailed information of datasets is shown in the Table \ref{tab:datasets_info}. 
 
\subsubsection{\textbf{Preprocessing}}
Following the common practice \cite{he2016fusing,wu2016collaborative}, we consider all numeric ratings (tagging behavior) as positive feedback. 
For both datasets, we group the interaction records by the user and order the sequence by interaction timestamps. 
For the Lastfm dataset, we combine multiple consecutive behaviors of the same user-item pair into one single interaction. 
To better reveal the sequential patterns encoded in the dataset, we follow the common practice \cite{rendle2010factorizing,kang2018self, zhang2019feature, sun2019bert4rec} and filter out users and items with less than $5$ interactions.
Table~\ref{tab:datasets_info} shows the statistics of the final dataset.

% \textcolor{red}{[ZHU: Movielens are originally dense so there is no need to remove infrequent items/users. However, for other datasets, they may not be reduced to 5-core (each user/item has at least 5 related items/users). The way we handle epinions is first removing infrequent users, and then replacing the infrequent items with a dummy item. Amazon datasets are better since they have 5-core reviews datasets, which we can treat the review as implicit feedback 1 and no review as 0. The problem of using Amazon data is that there are too many product categories that (1) the performance varies on different categories and (2) we may need to justify the use of one category.]}. 



\subsubsection{\textbf{Dataset Splitting}}\label{subsec:dataset_split}
We split the dataset into training and testing sets through the following steps. 
Given a user $u$'s complete viewing history $s=\{i_1,...,i_{q-1},i_q\}$, we retain the last item $i_q$ for the next-item evaluation task in testing and randomly split the remaining part into multiple continuous, non-overlapping subsequences $\{\{i_{1, 1},...,i_{1, m_1}\},... ,\{i_{k, 1}, \allowbreak ...,i_{k, m_k}\},\allowbreak ...\}$, where each subsequence's length $m_k$ is between $l_{min}$ and $l_{max}$.
For viewing history that is shorter than $l_{min}$, we prolong its length to $l_{min}$ through padding.
We set $l_{min} = 20$, $l_{max}=50$ for Lastfm and $l_{min} = 20$, $l_{max}=60$ for Movielens-1m, respectively. 
The last item $i_{k, m_k}$ of each subsequence is selected as the objective item $i_t$ during the training of \textit{IRN}. 
All subsequences of a user $u$ constitute the user's sequence set $S_u$, and the model training and validation are based on $S = \mathop{\bigcup}_{u=1}^{|U|} S_u$. 
To construct the testing set, we obtain the starting user behavior sequence $s_h=\{i_1, ..., i_{q-1}\}$ for each user. 
Based on the $s_h$ and an objective item $i_t$, each \textit{IRS} framework generates the influence path $s_p =\{i_j, i_{j+1}, ...\}$ following the process illustrated in Figure~\ref{fig:eval_setting}. 
We will further explain the criteria for choosing $i_t$ in Section \ref{subsec:objective_selection}.
Finally, we obtain a testing set of size $|U|$. 
It is worth noting that the test set does not contain ground-truth paths and each \textit{IRS} model generates influence paths based on the same test set independently.

% Note that each \textit{IRS} model generates the corresponding influence path based on the same $s_h$ and $i_t$ independently. 





\subsection{\textit{IRS} Evaluation}
\label{subsec:evaluation}
\subsubsection{\textbf{Objective Item Selection}}\label{subsec:objective_selection}
As introduced in previous sections, the objective item $i_t$ can influence the \textit{IRS}'s strategy when generating the influence path $s_p$. For the sake of fairness, for each $s_h$ in the testing set, we randomly sample an objective item $i_t$ from the whole item space based on the following criteria:
(1) $i_t \not\in s_h$. Under the problem formulation of \textit{IRS}, the objective should be a new item to the user.
(2) $i_t$ has at least $5$ interaction records. This prevents unpopular items from being selected as the objective item.%, which frequently results in decaying \textit{IRS} performance. 


\subsubsection{\textbf{Evaluation Metrics}}
Different from the traditional ``next-item'' \textit{RS} which only needs to evaluate the single recommended item based on a user's viewing history, \textit{IRS} has to evaluate the influence path (i.e., a sequence of recommended items), where both the user acceptance and the path's smoothness need to be taken into account. For example, a long influence path may turn out to be continuously related to the user's current interest but fail to reach the objective item, while a short influence path may recommend the objective item directly but deviates too much from the user's interest and is therefore rejected by the user. 

In order to measure a user's interest over the influence path $s_p$, or whether $s_p$ can better lead the user towards the objective item $i_t$, we need to estimate the joint probability $P(s_p|s_h)$ as well as the conditional probability $P(i_t|s_p)$. This can be formulated as a language model which defines the probability of each sequence appearing in a sequence corpora:
\begin{equation}
    \begin{aligned}
        P(i_1...i_q) =~& P(i_1)P(i_2|i_1)...P(i_q|i_{<q}) = \prod_{k=1}^qP(i_k|i_{<k})
    \end{aligned}
\end{equation}

For these concerns, we evaluate the influence path $s_p$ from two aspects: 
(1) whether the influence path $s_p$ can successfully shift the user interests towards the objective $i_t$,
and (2) whether $s_p$ satisfies the user's interest.
We design and employ the following metrics:
% \vspace{-1mm}
\begin{itemize}[leftmargin=0.4cm]
    \item \textbf{Success Rate ($SR_{M}$)} measures the ratio of generated $s_p$'s that can successfully reach the objective item $i_t$ within the maximum length $M$ (as denoted in Algorithm \ref{algo:ppath}):  
    \begin{equation}
        SR_{M} = \frac{1}{|U|}\sum_{u=1}^{|U|} 1(i_t^u \in s_p^u) 
    \end{equation}
    \item \textbf{Increase of Interest ($IoI_{M}$)} measures the change of user's interest in the objective item $i_t$ after being persuaded through $s_p$:
    \begin{equation}
        IoI_{M} = \frac{1}{|U|}\sum\limits_{u=1}^{|U|} \bigg(\log P(i_t^u|s_h^u \oplus s_p^u) - \log P(i_t^u|s_h^u) \bigg)
    \end{equation}
    where ``$\oplus$'' refers to the concatenation of two sequences; $P(i_t|s)$ is the probability that the objected item $i_t$ is accepted by a user with viewing sequence $s$. Here we use log form probability to avoid numerical underflow.
    \item \textbf{Increment of Rank ($IoR_{M}$)} measures the increase of the ranking for the objective item $i_t$ after being persuaded through $s_p$:
    \begin{equation}
        IoR_{M} = \frac{1}{|U|}\sum\limits_{u=1}^{|U|} -\bigg(R(i_t^u | s_h^u \oplus s_p^u) - R(i_t^u | s_h^u) \bigg)
    \end{equation}
    where $R(i_t^u | s_h^u)$ denotes the ranking of the objective item $i_t^u$ based on $P(i_t^u | s_h^u)$. 
    \item \textbf{Perplexity (PPL)} measures the naturalness and smoothness of the influence path $s_p$, that is, how likely the path can appear in the viewing history. In our experiment, PPL is defined as the conditional probability of that $s_p$ follows $s_h$: 
    \begin{equation}
        \begin{aligned}
            \mathrm{PPL}(s_p|s_h) = & \bigg( \prod_{k=1}^{|s_p|}P(i_k|s_h \oplus i_{<k}) \bigg)^{-\frac{1}{|s_p|}}\\
            \log(\mathrm{PPL}) = &\frac{1}{|U|}\sum_{u=1}^{|U|} \log \mathrm{PPL}(s_p^u|s_h^u)     \\
             = & \frac{1}{|U|}\sum_{u=1}^{|U|} \sum_{k=1}^{|s_p^u|}\log P(i_k^u|s_h^u \oplus i_{<k}^u)
        \end{aligned}
    \label{equ:n_gram}
    \end{equation}
    where $s_h \oplus i_{<k}$ denotes the concatenated sequence of the viewing history $s_h$ and the preceding items of $i_k$ in $s_p$, and $|s_p|$ denotes the length of $s_p$. Note that the logarithm form of perplexity is equivalent to the average of the log probability that the user accepts the path item $i_k$ in each step of the influence path. 
\end{itemize}

% In addition to evaluate the influencing power of the recommender, we employ the following metrics to assess the next-term interests match: 
% \begin{itemize}
%     \item \textbf{HR@20} (Hit Ratio) and \textbf{MRR} (Mean Reciprocal Rank) are two commonly used metrics in \textit{RS} literature. They measure whether the recommended item meets the user's \textit{current} interests \textit{without} considering any influence path $s_p$. They can be computed as: 
%     \begin{equation}
%     \begin{aligned}
%         HR@20 & =  \frac{1}{|U|}\sum_{u=1}^{|U|} 1\big(R(i_q^u | s_h^u) \leq 20 \big)\\
%         MRR & = \frac{1}{|U|}\sum_{u=1}^{|U|} \frac{1}{R(i_q^u | s_h^u)}\\
%     \end{aligned}
%     \label{eqn:hr20}
%     \end{equation}
%     where $|U|$ denotes the size of the test set, $s_h^u$ the viewing history sequence (not containing $i_q^u$) of user $u$, and $R(i_q^u | s_h^u)$ the ranking of item $i_q^u$ in each \textit{IRS}; $1(*)$ equals to $1$ if the condition ``$*$'' is true and $0$ otherwise. 
%     Recall that the last item ($i_q$) of the input sequence $\{i_1,...,i_{q-1},i_q\}$ is the labelled item.
% \end{itemize}

\subsubsection{\textbf{IRS Evaluator}}
As introduced above, the computation of $IoI_M$, $IoR_M$, and PPL relies on the term $P(i|s)$, which refers to the probability that item $i$ is accepted by a user given the viewing history $s$. This presents a unique challenge for the offline evaluation of \textit{IRS} with the logged dataset: many sequence-item interactions may not exist in the users' viewing histories, especially when the sequence $s$ is long. %Since the influence path $s_p$ can be composed of any number of any item, it makes it even more difficult to measure the user's response to the objective item $i_t$ after being persuaded through $s_p$. 

Traditional \textit{NLP} approaches estimate the term $P(i|s)$ by counting the occurrences of items as follows:
\begin{equation}
    P(i|s) = \frac{C(s \oplus i)}{C(s)}
\end{equation}
where $C(s)$ refers to the times that sequence $s$ occurs in the sequence corpora and $s \oplus i$ refers to the new sequence with $i$ appended into $s$. 
Due to the sparsity of \textit{RS} datasets, there can be many zero counts (i.e., $P(i|s)=0$) in computing the conditional probabilities, which makes the counting approximation approach ineffective. 

Inspired by the common practice of \textit{simulation based} experiments in reinforcement learning based \textit{RS} \cite{chen2019top, Huang_simulator2020, li2015counterfactual, huang2020keeping} and combinatorial recommendation \cite{yue2011linear, wang2019sequential}, we adopt an independent \textit{IRS} evaluator $\mathbb{E}$ to tackle the problem.
The evaluator $\mathbb{E}$ measures the relevance of item $i$ by estimating the probability of item $i$ following the sequence $s$, namely,
\begin{equation}
\label{eqn:evaluator}
    P(i|s) = \mathbb{E}(i, s)
\end{equation}
Specifically, we train an independent next-item recommender model which outputs a measurement for the probability term $P(i|s)$.
The recommender model $g$ contains a softmax layer which generates a probability distribution $\mathbf{D}$ over all items given an input sequence $s$. Finally, we compute $P(i|s)$ as:
\begin{equation}
\begin{aligned}
    \mathbf{D}(s) &= \mathbb{E}(s) = \mbox{Softmax}(g(s)) \\
    P(i|s) &= \mathbb{E}(i, s) = \mathbf{D}(s)[i]\\
\end{aligned}
\end{equation}
Although the evaluator is an approximation of real users, it provides a reasonably fair offline evaluation strategy for sequence-item interactions that do not appear in the dataset. 
% Note that the evaluator does not involve any user information and hence avoids the bias of favoring a specific \textit{RS}. 

An accurate evaluator should be capable of capturing the sequential patterns encoded in the viewing sequence and recommend the next item accurately. Therefore, we experiment with multiple state-of-the-art sequential recommenders and select the optimal one as the final evaluator. We measure the performance of the evaluator using \textbf{HR@20} (Hit Ratio) and \textbf{MRR} (Mean Reciprocal Rank):
% They measure whether the recommended item meets the user's \textit{current} interests \textit{without} considering any influence path $s_p$. 
% They can be computed as: 
\begin{equation}
\begin{aligned}
    HR@20 & =  \frac{1}{|U|}\sum_{u=1}^{|U|} 1\big(R(i_q^u | s_h^u) \leq 20 \big)\\
    MRR & = \frac{1}{|U|}\sum_{u=1}^{|U|} \frac{1}{R(i_q^u | s_h^u)}\\
\end{aligned}
\label{eqn:hr20}
\end{equation}
where $|U|$ denotes the size of the testing set, $s_h^u$ the viewing history sequence (not containing $i_q^u$) of user $u$, and $R(i_q^u | s_h^u)$ the ranking of item $i_q^u$ in each \textit{IRS}; $1(*)$ equals to $1$ if the condition ``$*$'' is true and $0$ otherwise. 
Recall that the last item ($i_q$) of the input sequence $\{i_1,...,i_{q-1},i_q\}$ is the labelled item. 

Specifically, we consider the following models for the \textit{IRS} evaluator:
\begin{itemize}[leftmargin=0.4cm]
    \item \textbf{GRU4Rec}~\cite{hidasi2018recurrent} employs the recurrent neural network (\textit{RNN}) based architecture to model user behavior sequences for sequential recommendation.  
    \item \textbf{Caser}~\cite{tang2018personalized} utilizes the convolutional neural network (\textit{CNN}) to learn the sequential patterns of user-item interactions in both horizontal and vertical way.
    \item \textbf{SASRec}~\cite{kang2018self} models the sequential dynamics of recommendation by using a self-attention-based model, which allows for capturing both long-term and short-term semantics. 
    \item \textbf{Bert4Rec}~\cite{sun2019bert4rec} further improves the user behavior sequences modeling with bidirectional self-attention and is considered one of the strongest baselines for the sequential recommendation.
\end{itemize}
The original models were implemented in various deep learning frameworks, and we port them to PyTorch based on the originally published code\footnote{https://github.com/graytowne/caser\_pytorch}\footnote{https://github.com/hidasib/GRU4Rec}\footnote{https://github.com/kang205/SASRec}\footnote{https://github.com/FeiSun/BERT4Rec}. We tune all hyperparameters of these models using the validation set and compare their results on the testing set. 



\begin{table}[tb]
\renewcommand{\arraystretch}{1.3}

    \centering
%     \setlength{\belowcaptionskip}{-5pt}
% 	\setlength{\abovecaptionskip}{3pt}
    \caption{Performance of IRS Evaluator. The bold number indicates the best performance and the underlined number indicates the second best performance. }
    % \resizebox{0.47\textwidth}{!}{
	\begin{tabular}{l|ll|ll}
		\hline
		\multirow{ 2}{*}{\diagbox{Method}{Dataset}}&\multicolumn{2}{c|}{Lastfm}&\multicolumn{2}{c}{Movielens-1M}\\ \cline{2-5}
	    Method&$HR@20$&$MRR$&$HR@20$&$MRR$\\ \hline\hline
	    {GRU4Rec}&0.0392&0.0081&0.243&\underline{0.063}\\ \hline
	    {Caser}&\underline{0.0460}&\underline{0.0106}&0.252&0.062\\ \hline
	    {SASRec}&0.0445&0.0097&\underline{0.257}&0.062\\ \hline
	    {Bert4Rec}&\textbf{0.0489}&\textbf{0.0199}&\textbf{0.264}&\textbf{0.076}\\ \hline
	\end{tabular}
% 	}
	\label{tab:evaluator}
% 	\setlength{\belowcaptionskip}{-10pt}
% 	\setlength{\abovecaptionskip}{-2pt}
% 	\vspace{-5mm}
\end{table}

Table \ref{tab:evaluator} shows the comparison results of \textit{IRS} evaluators. Among the tested sequential recommender models, \textit{Bert4Rec} has achieved the best performance in terms of all evaluation metrics, with around $4.5\%$ $HR@20$ and $58.4\%$ $MRR$ improvements against the second-best model. Therefore, \textit{Bert4Rec} is selected as the evaluator and used to provide a probability measure of $P(i|s)$ in the following experiment discussion. 




% Thus, we follow the common practice in \textit{NLP} \cite{bengio2003neural, celikyilmaz2020evaluation, gatt2018survey} to approximate the probability of a sequence using an \textit{n-gram} language model ($n=5$) with item embedding, which has been shown to be capable of capturing the semantic meanings of items~\cite{zhao2017ngram2vec}. 


% Notice that since most of the probabilities are small and multiplying multiple probabilities may lead to numerical underflow, all the probabilities are calculated in log form. 

% \subsubsection{N-grams} 
% The probability of the occurrence of an item $i$ given some history $h = \{i_1, i_2, ..., i_p\}$ can be estimated by counting the number of times that $h$ and $i$ occur in a large corpus, as follows:
% \begin{equation}
%     P(i|h) = \frac{C(h + i)}{C(h)}
% \end{equation}
% where $C$ is the counter function, $h + i$ means concating $h$ and $i$. Given an entire item sequence $\{i_1, i_2, ..., i_q\}$, the probability can be estimated using chain rule:
% \begin{equation}
% \begin{aligned}
%     P(i_1...i_q) =& P(i_1)P(i_2|i_1)P(i_3|i_1i_2)...P(i_q|i_1...i_{q-1})\\
%     =&\prod_{k=1}^qP(i_k|i_1...i_{k-1})
% \end{aligned}
% \end{equation}
% Instead of using the whole history in calculating the conditional probability, the n-grams approximate the history by considering the last $n-1$ words. For example, the bigram model makes the approximation $P(i_q|i_1...i_{q-1}) \approx P(i_q|i_{q-1})$ and the probability of an entire item sequence can be computed as:
% \begin{equation}
%     P(i_1...i_q) = \prod_{k=1}^qP(i_k|i_{k-1})
% \end{equation}
% For the general n-grams ($n \geq 2$), the probability of an entire item sequence can be computed as:
% \begin{equation}
%     P(i_1...i_q) = \prod_{k=1}^qP(i_k|i_{k-n+1}...i_{k-1})
%     \label{equ:n_gram}
% \end{equation}
% The bigram, trigram, 4-gram, and 5-gram are widely used to evaluate the sequences. 

% \subsection{IRS Evaluation}
% \subsubsection{Evaluation Metrics}
% \subsubsection{Results }



% In testing the model, we input $u$'s complete viewing history except $i_q$, $\{i_1, ..., i_{q-1}\}$, and a \textit{randomly} selected objective $i_t \not\in s$ to the model to generate the persuasion path $s_p$, where $i_q$ is retained for accuracy oriented metrics introduced in Section \ref{subsubsec:eval_accuracy}. The setup is illustrated in Figure \ref{fig:eval_setting}. 
% \noindent \textbf{Persuasion Path's Ability to Satisfy User Existing Interest:}
% \vspace{-1mm}




% \vspace{-1mm}
% \vspace{-1mm}



\begin{table*}[tb]
% 	\setlength{\belowcaptionskip}{-5pt}
% 	\setlength{\abovecaptionskip}{3pt}
\renewcommand{\arraystretch}{1.3}
	\caption{Comparison of various models on two datasets ($M = 20$). ``Vanilla'' means the original version of baselines, while ``Pf2Inf'' and ``Rec2Inf'' denote baselines that have been adapted to the IRS framework. The bold number indicates the best performance, and the underlined number indicates the second-best performance within IRS approaches. }
	\centering
% \resizebox{0.8\textwidth}{!}{
	\begin{tabular}{l|l||llll||llll}
		\hline
		\multicolumn{2}{c||}{\multirow{ 2}{*}{\diagbox{Method}{Dataset}}}&\multicolumn{4}{c||}{Lastfm}&\multicolumn{4}{c}{Movielens-1M}\\ \cline{3-10}
		\multicolumn{2}{c||}{}&$SR_{20}$&$IoI_{20}$&$IoR_{20}$&$\log$(PPL)&$SR_{20}$&$IoI_{20}$&$IoR_{20}$&$\log$(PPL)\\ \hline\hline
        \multirow{2}{*}{Pf2Inf}&Dijkstra& 0.031& 0.0192& 3.73 & 9.88 & 0.069 & 0.009 &362.8& 6.97\\ \cline{2-10}
        &MST& 0.0016& -0.0531& -11.5 & 8.13 & 0.031 & -0.026 &52.0& 8.47\\ \hline\hline
		\multirow{7}{*}{Vanilla}&POP& 0.00& -0.0119& 9.74 & 7.27 & 0.005 & -0.078 & 18.1 & 5.39\\ \cline{2-10}
		&BPR& 0.001& -0.123 & 5.57& 6.64 & 0.006 & -0.171 & 41.5 & 5.62\\ \cline{2-10}
		&TransRec& 0.00& -0.0720& -0.483& 6.69 & 0.005 & 0.083 & 19.9 & 5.11\\ \cline{2-10}
		&GRU4Rec& 0.001& -0.0818& 4.72 & 6.27 & 0.00 & -0.583 & -7.32 & 4.41 \\ \cline{2-10}
		&Caser& 0.002& 0.0110& 13.6 & 6.71& 0.00 & -0.887 & 7.36 & 3.78\\ \cline{2-10}
		&SASRec& 0.00& 0.0257& -15.0 & 6.36 & 0.001 & -0.003 & -0.918 & 3.95\\ \hline\hline
		\multirow{6}{*}{Rec2Inf}&POP& 0.0234& \underline{0.203} & 47.7 & 7.46  & 0.019 &  1.35 & 238.9 & 5.89 \\ \cline{2-10}
		&BPR& 0.0279 & -0.0218 & 41.9 & 6.80 & 0.021 & 0.930 & 242.8 & 6.01 \\ \cline{2-10}
		&TransRec& \underline{0.0625} & 0.0218 & \underline{48.9} & 6.77 & 0.042 & \underline{1.59} & 508.0 & 5.50\\ \cline{2-10}
		&GRU4Rec& 0.0140 & 0.0392 & 20.8 & \textbf{6.37} & 0.012 & 0.91 & 130.1 & 5.22 \\ \cline{2-10}
		&Caser& 0.0246 & 0.0236 & 15.82 & 6.81 & \underline{0.073} & 1.38 &  \underline{614.0} & \textbf{4.74} \\ \cline{2-10}
		&SASRec& 0.0137 & 0.0205 & 42.7 & 7.78& 0.014 & 1.10 & 139.8 & 6.03 \\ \hline
		\multicolumn{2}{c||}{IRN}& \textbf{0.142} & \textbf{0.572} & \textbf{160.7} & \underline{6.65} & \textbf{0.259} & \textbf{2.61} & \textbf{804.7} & \underline{4.94} \\ \hline
		
    	\end{tabular}
    % 	}
	\label{tab:random_result}
	%\vspace{-5pt}
\end{table*}


% \begin{table*}[tb]
% % 	\setlength{\belowcaptionskip}{-5pt}
% % 	\setlength{\abovecaptionskip}{3pt}
% \renewcommand{\arraystretch}{1.3}
% 	\caption{Comparison of various models on two datasets ($M = 20$). ``Vanilla'' means the original version of baselines, while ``Vec2Inf'' and ``Rec2Inf'' denote baselines that have been adapted to the IRS framework. The bold number indicates the best performance and the underlined number indicates the second best performance within IRS approaches. }
% 	\centering
% % \resizebox{0.8\textwidth}{!}{
% 	\begin{tabular}{l|l||llll||llll}
% 		\hline
% 		\multicolumn{2}{c||}{\multirow{ 2}{*}{\diagbox{Method}{Dataset}}}&\multicolumn{4}{c||}{Lastfm}&\multicolumn{4}{c}{Movielens-1M}\\ \cline{3-10}
% 		\multicolumn{2}{c||}{}&$SR_{20}$&$IoI_{20}$&$IoR_{20}$&$\log(PPL)$&$SR_{20}$&$IoI_{20}$&$IoR_{20}$&$\log(PPL)$\\ \hline\hline
% 		\multirow{7}{*}{Vanilla}&item2vec& 0.00& 0.00487& -13.1& 8.03& 0.001 & 0.360 & 2.78 & 5.74 \\ \cline{2-10}
% 		&POP& 0.00& -0.0119& 9.74 & 7.27 & 0.005 & -0.078 & 18.1 & 5.39\\ \cline{2-10}
% 		&BPR& 0.001& -0.123 & 5.57& 6.64 & 0.006 & -0.171 & 41.5 & 5.62\\ \cline{2-10}
% 		&TransRec& 0.00& -0.0720& -0.483& 6.69 & 0.005 & 0.083 & 19.9 & 5.11\\ \cline{2-10}
% 		&GRU4Rec& 0.001& -0.0818& 4.72 & 6.27 & 0.00 & -0.583 & -7.32 & 4.41 \\ \cline{2-10}
% 		&Caser& 0.002& 0.0110& 13.6 & 6.71& 0.00 & -0.887 & 7.36 & 3.78\\ \cline{2-10}
% 		&SASRec& 0.00& 0.0257& -15.0 & 6.36 & 0.001 & -0.003 & -0.918 & 3.95\\ \hline\hline
% 		Vec2Inf&item2vec& 0.008& 0.0139& 25.1 & 8.11 & 0.012 & 1.19 & 198.7 & 6.94 \\ \hline
% 		\multirow{6}{*}{Rec2Inf}&POP& 0.0234& \underline{0.203} & 47.7 & 7.46  & 0.019 &  1.35 & 238.9 & 5.89 \\ \cline{2-10}
% 		&BPR& 0.0279 & -0.0218 & 41.9 & 6.80 & 0.021 & 0.930 & 242.8 & 6.01 \\ \cline{2-10}
% 		&TransRec& \underline{0.0625} & 0.0218 & \underline{48.9} & 6.77 & 0.042 & \underline{1.59} & 508.0 & 5.50\\ \cline{2-10}
% 		&GRU4Rec& 0.0140 & 0.0392 & 20.8 & \textbf{6.37} & 0.012 & 0.91 & 130.1 & 5.22 \\ \cline{2-10}
% 		&Caser& 0.0246 & 0.0236 & 15.82 & 6.81 & \underline{0.073} & 1.38 &  \underline{614.0} & \textbf{4.74} \\ \cline{2-10}
% 		&SASRec& 0.0137 & 0.0205 & 42.7 & 7.78& 0.014 & 1.10 & 139.8 & 6.03 \\ \hline
% 		\multicolumn{2}{c||}{IRN}& \textbf{0.142} & \textbf{0.572} & \textbf{160.7} & \underline{6.65} & \textbf{0.259} & \textbf{2.61} & \textbf{804.7} & \underline{4.94} \\ \hline\hline
		
%     	\end{tabular}
%     % 	}
% 	\label{tab:random_result}
% 	%\vspace{-5pt}
% \end{table*}

\subsection{Baselines}
% \textcolor{red}{[ZHU: after doing some literature reviews, I remove TransUP and RNN, but add GRURec and Caser which are two state-of-the-art recsys that utilizes RNN/CNN. The baseliens can be categorized as (1) general method, (2) MC based method, and (3) NN based method.  ]}
% We compare our approach with \textbf{\textit{item2vec}}~\cite{barkan2016item2vec}, which is adapted to perform influential recommendation under the \textit{Vec2Inf} framework (see Section~\ref{subsec:vector}), and several baselines under the \textit{Rec2Inf} framework (see Section~\ref{subsec:rec2pros}). 
% We compare the model to the \textit{\textbf{VSPRS}} as introduced in Section \ref{subsec:vector}. \textit{VSPRS} is based on the well-known \textbf{\textit{item2vec}} model\cite{barkan2016item2vec}. We also compare our approach with several \textit{Rec2Pro}'s as introduced in Section \ref{subsec:rec2pros} modified from existing recommender systems as follows: 
We compare our approach with two path-finding algorithms under the \textbf{\textit{Pf2Inf}} framework and six \textit{RS} baselines under the \textbf{\textit{Rec2Inf}} framework. 
Overall, we use the following approaches as baselines:
\begin{itemize}[leftmargin=0.4cm]
    % \item \textbf{item2vec}~\cite{barkan2016item2vec} is a well-known embedding-based recommendation approach.
    \item \textbf{Dijkstra} finds the shortest path between two nodes in the item graph (described in Section \ref{subsec:pathfinding}). We select the influence path as the first $M$ items along the path from the last item in $s_h$ to $i_t$.
    \item \textbf{MST} constructs a minimum spanning tree from the constructed item graph. We select the influence path using the same process as \textit{Dijkstra}. 
    \item \textbf{POP} sorts all the items by occurrence and recommends the most popular items to the user. 
    \item \textbf{BPR}~\cite{rendle2012bpr} is a commonly used matrix factorization method that optimizes a pairwise objective function.
    % \item \textbf{FMC} uses Markov Chain to generate recommendation.
    % \item \textbf{FPMC}~\cite{rendle2010factorizing} adds personalization to \textit{FMC}.
    \item \textbf{TransRec}~\cite{he2017translation} models item-item and user-item translation relationships for large-scale sequential prediction.
    \item \textbf{GRU4Rec}~\cite{hidasi2018recurrent} is an \textit{RNN} based model for sequential recommendation.  
    \item \textbf{Caser}~\cite{tang2018personalized} is a \textit{CNN} based model for sequential recommendation. 
    \item \textbf{SASRec}~\cite{kang2018self} is a sequential recommender based on self-attention.
\end{itemize}

% For \textit{item2vec} under the \textit{Vec2Inf} framework, we use the recommended hyperparameters in the original implementation and set the item embedding dimension $d=20$ from $\{10, 20, 30, 40, 50\}$ and the distance threshold $\theta = 0.3$. 
For \textit{RS} approaches under the \textit{Rec2Inf} framework, we use the recommended hyperparameters in the original implementation and set the size of the candidate set $k=50$. We calculate the item distance using genre feature vector on Movielens-1m, and \textit{item2vec} \cite{barkan2016item2vec} embeddings on Lastfm, respectively.
% For baseline models 、under the \textit{Vec2Pro} and \textit{Rec2Pro} frameworks, we use the recommended hyperparameters in their original papers. 

\subsection{Experiment Result}
% \textcolor{red}{[ZHU: these parameters seem not important. Remove the discussion and replace it by the personalized factor]} Experiments show $d_{item}$ and $n_{l}$ significantly affect the model performance. \textcolor{red}{Rewrite this paragraph. The performance as well as the time consumed increases with larger $d_{item}$. Considering that the performance gain of incrementing $d_{item}$ from $30$ is negligible while the training time is prolonged, the optimal $d_{item}$ is set to $30$. It indicates that the context of an item can be well represented by a vector with size $30$. Similarly for $n_l$, the model optimizes considering the performance metrics and the efficiency when $n_l = 6$. Larger $n_{l}$ may enhance the model capacity in learning the complicated sequence patterns while the incurred complexity lay burden on the convergence and mitigate the positive effect.}

% For $w_{t}$ and $w_{h}$, they control the aggressiveness degree of model in approaching the objective item. \textcolor{red}{[Todo: graph and illustration]}.

% \begin{table*}[tb]
% % 	\setlength{\belowcaptionskip}{-5pt}
% % 	\setlength{\abovecaptionskip}{3pt}
% 	\caption{Comparison of various models on two datasets. ``Vanilla'' means the original version of baselines, while ``Vec2Pro'' and ``Rec2Pro'' denote baselines that have been adapted to the \textit{IRS} framework.}
% \resizebox{\textwidth}{!}{
% 	\begin{tabular}{ll|ll@{}l|l@{}|lllll@{}l@{}l|l}
% 		\hline
% 		\multirow{ 2}{*}{Datasets}&\multirow{ 2}{*}{Metrics}& \multicolumn{3}{c|}{Vanilla}&\multirow{1}{*}{Vec2Pro}&  \multicolumn{7}{c|}{Rec2Pro}&\multirow{2}{*}{IRN}\\ \cline{3-13}
% 		&&BPR&TransRec\;&Caser&item2vec\;&POP&BPR&FMC&FPMC&TransRec\;&SASRec\;&Caser&\\ \hline\hline
		
%         &$Hit@20$&0.169&0.176&0.162&0.103&0.074&0.168&0.154&0.116&0.176&0.147&0.161&\textbf{0.240}\\ \cline{2-14} 
% 	    &$MRR$&0.046&0.044&0.034&0.026&0.023&0.046&0.045&0.035&0.044&0.040&0.033&\textbf{0.067}\\ \cline{2-14} 
% 		\multicolumn{1}{c}{Lastfm-}
% 		&$SR_{20}$&0.008&0.016&0.002&0.039&0.038&0.038&0.086&0.037&0.082&0.041&0.042&\textbf{0.152}\\ \cline{2-14} 
% 		\multicolumn{1}{c}{1k} 
% 		&$IoI_{20}$&-0.083&-0.123&-0.566&0.738&0.453&0.300&1.01&0.642&0.570&0.92&-0.112&\textbf{1.53}\\ \cline{2-14}
% 		&$IoR_{20}$&19.2&26.5&-9.05&45.1&30.5&25.42&74.21&33.9&46.3&61.3&50.13&\textbf{200.0}\\ \cline{2-14} 
%         &$\log(PPL)$&&&&&&&&&&&&\\ \hline\hline
		
%         &$Hit@20$&0.095&0.080&0.252&0.056&0.042&0.094&0.064&0.048&0.073&0.137&0.250&0.242\\ \cline{2-14} 
%         &$MRR$&0.030&0.024&0.063&0.017&0.013&0.029&0.019&0.013&0.017&0.031&0.061&\textbf{0.073}\\ \cline{2-14} 
% 		\multicolumn{1}{c}{Movielens}
% 		&$SR_{20}$&0.005&0.005&0.00&0.012&0.019&0.020&0.017&0.010&0.011&0.014&0.061&\textbf{0.259}\\ \cline{2-14} 
% 		\multicolumn{1}{c}{1M}
% 		&$IoI_{20}$&-0.267&0.102&-1.35&1.39&1.60&1.51&1.82&0.67&0.56&1.10&1.34&\textbf{2.60}\\ \cline{2-14}
% 		&$IoR_{20}$&6.43&-17.6&4.38&198.7&262.8&255.9&204.4&87.3&128.5&139.8&650.0&\textbf{804.7}\\ \cline{2-14} 
% 		&$\log(PPL)$&5.80&5.50&3.80&6.94&6.28&6.36&6.71&6.30&5.74&6.03&4.65&4.95 \\ \hline

% % 		\multicolumn{1}{|c|}{}         &$Hit@20$&&0.050&0.067&0.188&0.211&0.227&&0.298&0.241\\ \cline{2-11} 
% % 		\multicolumn{1}{|c|}{}         &$MRR$&&0.015&0.022&0.093&0.094&0.089&0.101&0.092&0.169\\ \cline{2-11} 
% % 		\multicolumn{1}{|c|}{Lastfm}   &$IoI_{20}$&&0.717&0.516&0.013&0.107&-0.003&0.097&0.190&0.304\\ \cline{2-11}
% % 		\multicolumn{1}{|c|}{1k}       &$IoR_{20}$&&1327.5&1131.2&&&&&&650.3\\ \cline{2-11} 
% % 		\multicolumn{1}{|c|}{}         &$SR_{20}$&&0.001&0.002&&&&&&0.004\\ \cline{2-11} 
% % 		\multicolumn{1}{|c|}{}         &$PPL$&&6.86&6.71&&&&&&6.212\\ \cline{1-11} 
% 	\end{tabular}}
% 	\label{tab:random_result}
% 	%\vspace{-5pt}
% \end{table*}

% \begin{table*}[tb]
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|l|l||l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{ 2}{*}{Datasets}&\multirow{2}{*}{Methods}&\multirow{1}{*}{Vec2Pro}&  \multicolumn{2}{|c|}{POP}&\multicolumn{2}{|c|}{BPR}&\multicolumn{2}{|c|}{FMC}&\multicolumn{2}{|c|}{FPMC}&\multicolumn{2}{|c|}{TransRec}&\multicolumn{2}{|c|}{SASRec}&\multicolumn{2}{|c|}{Caser}&\multirow{2}{*}{PRN}\\ \cline{3-17}
% &&item2vec&Origin&Pro.&Origin&Pro.&Origin&Pro.&Origin&Pro.&Origin&Pro.&Origin&Pro.&Origin&Pro.&\\ \hline\hline

% &$Hit@20$&0.103&0.086&0.086&&0.168&&0.154&&0.116&&0.176&&0.147&&0.161&\textbf{0.213}\\ \cline{2-18} 
% &$MRR$&0.026&0.022&0.021&&0.046&&0.045&&0.035&&0.044&&0.040&&0.033&\textbf{0.050}\\ \cline{2-18} 
% {Movielens}
% &$SR_{20}$&0.039&0.008&0.038&0.008&0.038&0.008&0.086&0.006&0.037&0.016&0.082&&0.041&0.002&0.042&\textbf{0.152}\\ \cline{2-18} 
% {100k}
% &$IoI_{20}$&0.738&0.331&0.453&-0.083&0.300&0.298&1.01&0.108&0.642&-0.123&0.570&&0.92&-0.566&-0.112&\textbf{1.53}\\ \cline{2-18}
% &$IoR_{20}$&45.1&6.46&30.5&19.2&25.42&25.8&74.21&3.13&33.9&26.5&46.3&&61.3&-9.05&50.13&\textbf{200.0}\\ \cline{2-18} 
% &$PPL$&6.71&5.80&6.42&5.50&6.40&5.83&6.55&5.74&6.59&5.02&6.05&&5.98&4.68&5.32&5.36\\ \hline\hline


% &$Hit@20$&0.056&0.043&0.042&&0.095&&0.064&&0.048&&0.073&&0.137&&\textbf{0.252}&0.230\\ \cline{2-18} 
% &$MRR$&0.017&0.010&0.010&&0.029&&0.019&&0.013&&0.023&&0.031&&0.063&\textbf{0.071}\\ \cline{2-18} 
% {Movielens}
% &$SR_{20}$&0.012&0.004&0.019&0.005&0.020&&0.017&&0.010&&0.011&&0.014&&0.061&\textbf{0.259}\\ \cline{2-18} 
% {1M}
% &$IoI_{20}$&1.39&0.107&1.60&-0.267&1.51&&1.82&&0.67&&0.56&&1.10&&1.35&\textbf{2.60}\\ \cline{2-18}
% &$IoR_{20}$&198.7&-11.2&262.8&6.43&255.9&&204.4&&87.3&&128.5&&139.8&&650.0&\textbf{804.7}\\ \cline{2-18} 
% &$PPL$&6.94&5.73&6.28&5.80&6.36&&6.71&&6.30&&5.74&&6.03&&\textbf{4.65}&4.95 \\ \hline
% \end{tabular}}
% \caption{Overall Comparison\gu{too short caption?}}
% \label{tab:random_result}
% \vspace{-5mm}
% \end{table*}

\subsubsection{\textbf{Overall Comparison}}
\label{subsubsec:overall_comp}
Table \ref{tab:random_result} shows the overall results of various models on the two datasets. As we can see, \textit{IRN} significantly outperforms other baselines in terms of $IoI_{20}$, $IoR_{20}$, and $SR_{20}$ on both datasets. 
In the Lastfm dataset, $14.2\%$ of the influence paths generated by \textit{IRN} for the testing set can reach the objective item within $20$ steps.
In the Movielens-1M dataset, $25.9\%$ of testing sequences can successfully lead to the objective item, while the strong baseline method \textit{Caser} can only achieve 7.3\%. 
In terms of PPL, \textit{IRN} achieves the second best results, only next to \textit{TransRec} in Lastfm and \textit{Caser} in Movielens-1m, respectively. 
It indicates that \textit{IRN} does not hamper the smoothness of the influence path while achieving superior influencing performance. 
Note that a trade-off exists between the influencing power of the recommender and the smoothness of the influence path. We will further discuss the aggressiveness of \textit{IRS} in Section \ref{subsubsec:aggressive_pers}.

In comparison, \textit{Dijkstra} under the \textit{Pf2Inf} framework achieves greater influencing performance at the cost of high PPL. This indicates that although path-finding algorithms manage to find a path from the viewing history to the objective, it often fails to satisfy the user's current interests and is likely to be rejected by users in the middle of persuasion. 
We also compare \textit{IRN} with the vanilla versions (i.e., the original model without being adapted to the \textit{Rec2Inf} paradigm) of baselines. 
The influence path $s_p$ of each vanilla model is generated by repeatedly recommending the item with the maximum $P(i|s)$.
Since the vanilla model is driven solely by users' current interest, we can observe a $SR_{20}$ and $IoI_{20}$ approximately equal to zero for most vanilla baselines.
Compared to their vanilla versions, these adapted baselines can achieve a higher $SR_{20}$ and have a  significantly larger $IoI_{20}$ and $IoR_{20}$, which indicates that the \textit{Rec2Inf} frameworks are effective in increasing the user's interest in the objective item. 
However, the adapted baselines generally have a higher PPL. 
It is reasonable because they need to pay extra attention to the objective item at each step of the influence path, frequently resulting in a recommendation that suits the user's interest less. 

In summary, \textit{IRN} outperforms the baselines in most evaluation metrics, which validates its capability of generating natural and smooth influence paths.

% The first task that the recommended items in the \textit{Persuasion Path} should satisfy the current user interests can be evaluated by the following three metrics: $Hit@20$, $MRR$, and $PPL$. For traditional metrics $Hit@20$ and $MRR$, the last item $i_q$ in the real viewing history is remained and they measure how the first item in the \textit{Persuasion Path} meets the current user interests. The \textit{PRN} has outperformed most other baselines despite that it has smaller $MRR$ on Movielens-1m compared to \textit{TransRec} and the statistics may be slightly smaller than those reported in the state-of-the-art deep learning papers. It is reasonable since the \textit{PRN} may recommend a less welcomed item if the objective item is far away from the current user interests, which results in sacrificing precision of current interests for persuasion capacity. 

% For the perplexity $PPL$ calculated by the evaluator, the \textit{PRN} has outperformed all the baselines, which indicates that the \textit{Persuasion Path} generated by \textit{PRN} is more natural and easier to accept by the users. \textcolor{red}{[Todo: evaluate \textit{MPRS}]} Notice that the \textit{POP} model which recommends the most popular items among all the users can have smaller $PPL$ despite it has worse $Hit@20$ and $MRR$. After investigation into its \textit{Persuasion Path}, we find that the path contains popular items can be regarded as more natural by the evaluator. For the most extreme case which does not occur in the experiment, the path $\{i_{pop}, i_{pop},..., i_{pop}, i_{pop}\}$ which simply repeats the most popular item $i_{pop}$ in Movielens-100k has $PPL = 5.81$. 

% The second task that the \textit{Persuasion Path} successfully should lead to the objective item can be evaluated using the other three metrics: $IoI_{20}$, $IoR_{20}$, and $SR_{20}$. For the successful rate $SR_{20}$, it calculates the ratio of paths that reach the objective items with maximum path length $20$. Since $20$ may not be adequate for most \textit{PRS} to reach a random objective item, most methods have rather small $SR_{20}$. Still the \textit{PRN} has significantly outperformed other baselines on all the three datasets. Even though the \textit{Persuasion Path} may not successfully end at the objective item, it may shift the user interests toward the objective, which can be estimated by $IoI_{20}$ and $IoR_{20}$. \textcolor{red}{[Todo: compare the two metrics]}

% \textcolor{red}{[ZHU: contents to be included in the overall discussion: (1) compare the property of dataset (size, density) (2) compare the \textit{MPRS} themselves (3) discuss the balance between two tasks]}


\subsubsection{\textbf{Short-term Interests Match}}
% \textit{IRN} has achieved comparable performance regarding $Hit@20$ and $MRR$, which shows that \textit{IRN} can lead users' interests towards the objective item without sacrificing much accuracy on modeling their existing interests.
In addition to evaluating the influencing power of the recommender models, we also investigate whether they can achieve comparable performance in the task of traditional next-item recommendation. 

Table \ref{tab:short-term} displays the performance of various models in terms of next-item recommendation. 
In general, baseline models under the \textit{IRS} framework achieve suboptimal performance compared to the state-of-the-art next-item recommenders. 
We also observe a $2 \sim 20\%$ performance loss compared to their vanilla versions under the \textit{Rec2Inf} framework. 
% This is reasonable since \textit{IRS} trades part of the next-item recommendation accuracy for the ability of performing influencing recommendation. 
The reason could be that the \textit{IRS} needs to shift towards the objective $i_t$ early if $i_t$ is far from the user's current interest. This cause the model to recommend an unfamiliar item to the user, thus reducing the recommendation accuracy. 
Yet \textit{IRN} achieves comparable results with respect to $Hit@20$ and $MRR$ on the two datasets, with around $9.0\%$ $HR@20$ and $9.2\%$ $MRR$ performance loss compared to the best-performed $Bert4Rec$. This indicates that even with the objective item $i_t$, \textit{IRN} can still capture the user's current interests without abruptly heading for $i_t$. 

\begin{table}[tb]
\renewcommand{\arraystretch}{1.3}

%     \setlength{\belowcaptionskip}{-5pt}
% 	\setlength{\abovecaptionskip}{3pt}
    \caption{Performance of IRS in terms of next-item recommendation.}
    \renewcommand{\arraystretch}{1.3}

    % \resizebox{0.48\textwidth}{!}{
	\begin{tabular}{l|ll|ll|ll}
		\hline
		\multicolumn{3}{c|}{\multirow{ 2}{*}{\diagbox{Method}{Dataset}}}&\multicolumn{2}{c|}{Lastfm}&\multicolumn{2}{c}{Movielens-1M}\\ \cline{4-7}
	    \multicolumn{3}{c|}{}&$HR@20$&$MRR$&$HR@20$&$MRR$\\ \hline\hline
	    
	    &&{GRU4Rec}&0.0392&0.0081&0.243&0.063\\ \cline{2-7}
	    Next-item&&{Caser}&0.0460&0.0106&0.252&0.062\\ \cline{2-7}
	    RS&&{SASRec}&0.0445&0.0097&0.257&0.062\\ \cline{2-7}
	    &&{Bert4Rec}&0.0489&0.0199&0.264&0.081\\ \hline\hline
	    
	    \multirow{4}{*}{IRS}&&{GRU4Rec}&0.0387&0.0079&0.198&0.047\\ \cline{2-7}
	    &&{Caser}&0.0430&0.0102&0.250&0.061\\ \cline{2-7}
	    &&{SASRec}&0.0437&0.0092&0.207&0.041\\ \cline{2-7}
	    &\multicolumn{2}{c|}{IRN}&0.0458&0.0190&0.242&0.073\\ \hline\hline
	\end{tabular}
% 	}
	\label{tab:short-term}
% 	\setlength{\belowcaptionskip}{-10pt}
% 	\setlength{\abovecaptionskip}{-2pt}
% 	\vspace{-5mm}
\end{table}

% \begin{table}[tb]
% \renewcommand{\arraystretch}{1.3}

% x%     \setlength{\belowcaptionskip}{-5pt}
% % 	\setlength{\abovecaptionskip}{3pt}
%     \caption{\textit{IRS} Performance in terms of Short-term Interests Match. }
%     \renewcommand{\arraystretch}{1.3}

%     % \resizebox{0.48\textwidth}{!}{
% 	\begin{tabular}{l|ll|ll|ll}
% 		\hline
% 		\multicolumn{3}{c|}{\multirow{ 2}{*}{\diagbox{Method}{Dataset}}}&\multicolumn{2}{c|}{lastfm}&\multicolumn{2}{c}{Movielens-1M}\\ \cline{4-7}
% 	    \multicolumn{3}{c|}{}&$HR@20$&$MRR$&$HR@20$&$MRR$\\ \hline\hline
	    
% 	    &\multicolumn{2}{c|}{GRU4Rec}&&&0.243&0.063\\ \cline{2-7}
% 	    Next-item&\multicolumn{2}{c|}{Caser}&&&0.252&0.062\\ \cline{2-7}
% 	    RS&\multicolumn{2}{c|}{SASRec}&&&0.257&0.062\\ \cline{2-7}
% 	    &\multicolumn{2}{c|}{Bert4Rec}&&&\textbf{0.264}&\textbf{0.081}\\ \hline\hline
	    
% 	    \multirow{4}{*}{IRS}&\multirow{3}{*}{Rec2Pro}&{GRU4Rec}&&&0.198&0.047\\ \cline{3-7}
% 	    &&{Caser}&&&0.250&0.061\\ \cline{3-7}
% 	    &&{SASRec}&&&0.137&0.031\\ \cline{2-7}
% 	    &\multicolumn{2}{c|}{IRN}&&&0.242&0.073\\ \hline\hline
% 	\end{tabular}
% % 	}
% 	\label{tab:short-term}
% % 	\setlength{\belowcaptionskip}{-10pt}
% % 	\setlength{\abovecaptionskip}{-2pt}
% % 	\vspace{-5mm}
% \end{table}


\begin{figure}[tb]
% 	\setlength{\belowcaptionskip}{-5pt}
% 	\setlength{\abovecaptionskip}{3pt}
	\centering
	\includegraphics[width=0.47\textwidth]{step.png}
	\caption{Success rate $SR_M$ versus path length $M$.}
	\label{fig:step}
% 	\vspace{-5mm}
\end{figure}

\subsubsection{\textbf{Aggressiveness of IRS}}
\label{subsubsec:aggressive_pers}
One notable phenomenon observed in Section~\ref{subsubsec:overall_comp} is that
%In Section~\ref{subsubsec:overall_comp} we set the maximum persuasion path length $M$ to 20, and we can see 
even though \textit{IRN} significantly outperforms the baselines, the majority of the generated influence paths cannot successfully end at the objective item (e.g., $SR_{20}$ is only 14.2\% and 25.9\% on the two datasets, respectively). 
In this section, we study this phenomenon by analyzing the aggressiveness of influence paths. We hypothesize that whether $s_p$ can reach the objective item is mainly influenced by two factors: the maximum path length $M$ and the \textit{Aggressiveness Degree} (\textit{AD}) of each \textit{IRS}.
Hence, we investigate the relation between these two factors and the success rate of reaching the objective item ($SR$).

Figure~\ref{fig:step} illustrates the relationship between the maximum path length and the success rate. For clarity, we only compare \textit{IRN} to the strong baselines in the \textit{Rec2Inf} framework. 
In general, for all methods, the success rate increases as $M$ increases since longer influence paths increase the chance of reaching the objective. In addition to the outstanding performance, \textit{IRN} achieves a steady improvement of $SR$ as the influence path length increases, whereas the baselines' $SR$ quickly flattens out to a low level. This can be attributed to the fact that \textit{IRN} incorporates the objective item in the training process, thus enabling long-range planning in the influencing process. In contrast, the baseline models make an influential recommendation at each step independently and locally.

% As $d$ increases, the percentage of the path generated by the $PRN$ reaching the target item grows steadily, and have achieved $0.35$ in Movielens-100k and $0.49$ in Movielens-1m given $d=50$. In comparison, despite that $Rec2Pros$ models also benefit from increase of $d$, the growth rate is much smaller and most of them end at $SR_{50} < 0.1$.



Figure~\ref{fig:aggressive} illustrates the impact of aggressiveness degree (\textit{AD}) when \textit{IRS} is approaching the objective item. Each recommender has its own parameters to control the \textit{AD}. As we can see, \textit{AD} for the baselines is correlated to the size of the candidate set $k$. As introduced in Section \ref{subsec:rec2pros}, the \textit{Rec2Inf} framework selects the item that is closest to the objective from the top $k$ candidate set. When $k=1$, this is equivalent to the original recommender system which simply predicts the next item without considering the objective. When $k$ is set to the total number of items, it may recommend the objective item directly which has zero distance to itself. 
Different from the baselines, \textit{AD} for \textit{IRN} is related to the objective mask weight $w_t$. Larger $w_t$ enforces the model to rely more on the objective item in the recommendation. 

In order to compare \textit{AD}'s influence to baselines and \textit{IRN}, we need to unify \textit{AD}'s of different methods to the same scale. Therefore, we set 5 levels of $k = \{10,20,30,40,50\}$ for \textit{Rec2Inf} baselines and 5 levels of $w_t = \{0, 0.25, \allowbreak 0.5, 0.75, 1\}$ for \textit{IRN}, both 5 levels are then mapped as the x-axis of Figure \ref{fig:aggressive}. 
Figures~\ref{fig:aggressive}(a) and (b) show the value of $SR_{20}$ under different levels of \textit{AD}s. As expected, when \textit{AD} increases, $SR_{20}$ increases accordingly since more attention on the objective item can increase the chance of reaching the objective. In addition, \textit{IRN} significantly outperforms the baselines given the same \textit{AD}. This indicates that the model is effective in leading users towards the objective. 
Figures~\ref{fig:aggressive}(c) and (d) depict the perplexity over different levels of \textit{AD}s. A higher perplexity indicates a lower likelihood that users accept the influence paths. As we can see, most baseline methods exhibit a clear trade-off between $SR_{20}$ and PPL (higher $SR$ tends to have low PPL), probably because the aggressive influencing strategy increases the abruptness of sequential recommendation. 
In contrast, \textit{IRN} is superior to other models with a significantly higher $SR_{20}$ and a smaller PPL, demonstrating its capability of effectively leading users towards the objective and maintaining a high level of smoothness.
% in recommending valid sequential items under different \textit{AD}s consistently.
Furthermore, we observe that there does not exist a universal optimal \textit{AD} which can achieve the best $SR_{20}$ and PPL simultaneously. This indicates that the selection of \textit{AD} in the \textit{IRS} framework should be adapted to the requirement of the applications.
\begin{figure}[tb]
% 	\setlength{\belowcaptionskip}{-5pt}
% 	\setlength{\abovecaptionskip}{3pt}
	\centering
	\includegraphics[width=0.47\textwidth]{aggressive.png}
	\caption{Performance of \textit{IRS} under different aggressiveness degrees.}
	\label{fig:aggressive}
\end{figure}

\subsubsection{\textbf{Effectiveness of the Personalized Mask Weight}}
\label{subsubsec:personalize_mask_weight}

\begin{figure}[tb]
% 	\setlength{\belowcaptionskip}{-5pt}
% 	\setlength{\abovecaptionskip}{3pt}
	\centering
	\includegraphics[width=0.47\textwidth]{distribution.png}
	\caption{Distribution of the \textit{Personalized Impressionability Factor}.}
	\label{fig:distribution}
% 	\vspace{-5pt}
\end{figure}

\begin{table}[tb]
% 	\setlength{\belowcaptionskip}{-5pt}
% 	\setlength{\abovecaptionskip}{3pt}
\renewcommand{\arraystretch}{1.3}

	\caption{Comparison of Different Masks.}
% \resizebox{0.47\textwidth}{!}{
    \centering
	\begin{tabular}{l|l@{}ll|l@{}ll}
		\hline
		\multirow{ 2}{*}{Mask Type}&\multicolumn{3}{c|}{Lastfm}&\multicolumn{3}{c}{Movielens-1M}\\ \cline{2-7}
	    &$\log(PPL)$\;&$SR_{20}$&$IoI_{20}$&$\log(PPL)$\;&$SR_{20}$&$IoI_{20}$\\ \hline\hline
	    {Type 1}&5.93&0.002&0.011&4.27&0.009&0.054\\ \hline
	    {Type 2}&6.55&0.118&0.477&4.92&0.232&2.01\\ \hline
	    {Type 3}&6.65&0.142&0.572&4.94&0.259&2.61\\ \hline
	\end{tabular}
% 	}
	\label{tab:compare_mask}
% 	\vspace{-5pt}
\end{table}

As introduced in Section~\ref{subsec:sprs}, The \textit{Personalized Impressionability Mask} (\textit{PIM}) models a user's personal impressionability about the persuasion. Table \ref{tab:compare_mask} compares the performance of various masking schemes. In ``Type 1'' the model will not pay extra attention to the objective (i.e., $w_h=w_t=0$), in ``Type 2'' the objective has a uniform large weight ($w_t=1$), and in ``Type 3'' the model integrates the \textit{Personalized Impressionability Factor} $r_u$ and the objective has weight $r_uw_t$. Compared to ``Type 1'', ``Type 2'' has significantly improved the user's acceptance of the objective item (measured by $IoI_{20}$ and $SR_{20}$) at the expense of the smoothness of the path (measured by $\log(PPL)$). The addition of $r_u$ further increases the influence performance by approximately $20\%$ without evident impact to the smoothness. 

The \textit{IRN} learns $r_u$ for each user. We further investigate the distribution over $r_u$ values, as shown in Figure \ref{fig:distribution}. A larger $r_u$ indicates that the user is more adventurous and prefers a larger \textit{AD}. Thus, recommended items by \textit{IRN} are more close to the objective. On the other hand, a smaller $r_u$ results in recommendations that depend more on the user's historical interests. In general, $r_u$ follows a normal distribution on both datasets. This validates our intuition that users are indeed different in accepting influential recommendations and that \textit{PIM} is effective in modeling their different personalities.

\subsubsection{\textbf{Stepwise evolution of User Interests}} 
To get a deeper insight into the influencing process, we study the evolution of the influence path in each step. This gives us a micro view of how \textit{IRS} leads the user towards the objective. 
Specifically, we analyze two probabilities, namely, the ``objective probability'' $P(i_t|s_h\oplus i_{<k})$ (i.e., the probability that the user likes objective item $i_t$ at the $k^{th}$ influencing step) and ``item probability'' $P(i_k|s_h\oplus i_{<k})$ (i.e., the probability that the user is satisfied with item $i_k$ at the $k^{th}$ influencing step) over all the influence paths, which can be calculated using the \textit{IRS} evaluator $\mathbb{E}$. 
To facilitate analysis, we average the two probabilities on the testing sequences.  
Note that influence paths may have various lengths due to early reach to the objective, which affects the averaging of $P(i_t|s_h\oplus i_{<k})$ and $P(i_k|s_h\oplus i_{<k})$. Therefore, we exclude early-success paths which account for only a small fraction given $M=20$. 

Figure \ref{fig:grad} presents the results of stepwise user interests evolution.
On both datasets, the influence paths generated by \textit{IRN} can lead the user towards the objective steadily while maintaining a high probability to be accepted by the user. 
In comparison, influence paths recommended by most adapted baselines cannot steadily lead users to the objective, as evident from their flat curves. 
In the Movielens-1m dataset, the suboptimal approach \textit{Caser} also demonstrates a steadily increasing probability curve of the user accepting the objective item, but the increase amplitude is far below \textit{IRN}. 
Experiment results show that \textit{IRN} can consistently utilize the sequential dependence signals accumulated throughout the evolution of the influence path.


% In comparison, most baselines' influence paths cthe\gu{?} sequential dependencies accumulated through the evolution of path while the baselines cannot.
% For example, the path with length $10$ participates in the first $10$ steps while it is omitted in the next $10$ steps, which may skew up the average probability terms in the first $10$ steps. 

\begin{figure}[tb]
	%\setlength{\belowcaptionskip}{-5pt}
% 	\setlength{\abovecaptionskip}{3pt}
	\centering
	\includegraphics[width=0.47\textwidth]{grad.png}
	\caption{Stepwise evolution of user interests. (a) and (b) display the change of the objective probability as the influence path extends. (c) and (d) display the change of item probability through the path.}
	\label{fig:grad}
\end{figure}


% \subsubsection{\textbf{Effect of the Objective Item}}
% \label{subsubsec:objective}
% We investigate the effect of different objective items on influencing recommendation. 
% Intuitively thinking, if the objective is set to an item that is close to the user’s interest, the success rate can be high and vice versus. 
% We measure the proximity of the objective item $i_t$ to the user using the item embedding distance $d(i_t, s_h)$ between $i_t$ and the average of user’s history items. 
% For each testing sequence, we select the 
% We calculate the distance based on genre feature vector on Movielens-1m and normalized \textit{item2vec} embeddings on Lastfm. 

% Figure \ref{fig:objective} displays the results.  
% For \textit{IRN} and \textit{Transrec}, more than $50\%$ of the influence paths in the testing set can achieve the objective within 20 step when $\mu = 0.25$. In contrast, the topped-performed \textit{IRN} can achieve only $-$ and $-$ $SR_{20}$ on Lastfm and Movielens-1m, respectively. 
% In general, all the approaches have a decreasing success rate as the more unfamiliar item is selected as the objective. \textcolor{red}{Todo: considering changing the way of representing distance between objective and user;}

% \begin{figure}[tb]
% % 	\setlength{\belowcaptionskip}{-5pt}
% % 	\setlength{\abovecaptionskip}{3pt}
% 	\centering
% 	\includegraphics[width=0.47\textwidth]{objective.png}
% 	\caption{Effect of Objective Item on Influencing Recommendation. \textcolor{red}{Todo}}
% 	\label{fig:objective}
% % 	\vspace{-5mm}
% \end{figure}

% have minimal persuasion effect on Movielens-100k. Regarding Movielens-1m, even though some $Rec2Pros$ can capture the user interests quickly at the beginning, it is at the cost of low $P(i_k|h)$ and they cannot guarantee a steady growth of $P(i_t|h)$. Notice that without considering the early success paths, \textit{CASER} has comparable performance to \textit{PRN} with smaller $P(i_t|h)$ and higher $P(i_k|h)$.

% In conclusion, by analyzing the stepwise evolution of user interests, we show that the \textit{PRN} is able to smoothly lead the user to the target item. 

% Figure \ref{fig:grad}(a) display one local example of the stepwise user interests in the target item. At the beginning, the user is not interested in the target item with the log probability slightly below $-13$ at $step = 0$.  Along with the extension of recommendation path, the user interests in the target item gradually increase, and ends up with log probability estimated $-10.5$ at $step=30$. Similarly, Figure \ref{fig:grad}(b) averages the log probability terms which measure the user interests in the target item over all the testing samples at each step. Despite the oscillating progress, we can observe clear increasing pattern of user interests in target items versus the extension of path, which indicates that the PRS is capable of persuading the user to accept the target item. 

% Figure \ref{fig:grad}(c)(d) display the local example and the globally average result of the user interests in the recommended items, respectively. The horizontal dashed line refers to the average accept probability $p_{avg}$ over all the items. As shown in the two subfigures, the probability terms of the user to accept recommended items are significantly higher than $p_{avg}$, which indicates that the recommended items match the current interests of users. On the other hand, the accept probability curve is rather smooth. The user will not feel incongruent with the recommended items, which avoids the possible failure that the user leaves at the early step in the recommendation path.


\subsubsection{\textbf{Hyperparameter Tuning and Ablation Study}}
We run \textit{IRN} with different combinations of hyperparameter settings and find the optimal group of parameters using grid search. We optimize \textit{IRN} using the Adam algorithm with a dynamic learning rate scheduler which reduces the learning rate by a factor of $2$ once the learning stagnates. 

The ranges and optimal values of the hyperparameters are shown in Table~\ref{tab:hyper}. %We set the maximum and minimum sequence lengths to $30$ and $20$, respectively. For other parameters, 
$l_{min}$ and $l_{max}$ refer to the minimum and maximum sequence lengths related to the dataset splitting as introduced in Section \ref{subsec:dataset_split}.
$lr$ denotes the starting learning rate for the model which ranges from $1e-4$ to $1e-2$.
$d$ denotes the embedding size of items, while $d'$ denotes the embedding size of users. $L$ denotes the number of decoder layers, $h$ denotes the number of heads for attention, and $w_t$ is related to the weight of the attention mask for the objective item. 
With the optimal setting of hyperparameters, the training of \textit{IRN} takes approximately 1 hour on Lastfm and 2 hours on Movielens-1M, respectively, using a machine with one GTX-2080Ti GPU. 
In terms of scalability, the computational perplexity of \textit{IRN} is $\mathcal{O}(m^2d + |I|d)$ where $m$ and $I$ refer to the input length and the item set, respectively. 
The framework can be easily paralleled to multiple GPUs to accelerate the computation without significantly affecting the performance. 



\begin{table}[tbp]
% 	\setlength{\belowcaptionskip}{-5pt}
% 	\setlength{\abovecaptionskip}{3pt}
\renewcommand{\arraystretch}{1.3}

    \caption{Hyperparameter Settings}
    \centering
    % \resizebox{0.35\textwidth}{!}{
    \begin{tabular}{llll}
    \toprule
    Name&Range&Lastfm&Movielens-1m\\
    \midrule
    $l_{max}$& [30, 40, 50, 60, 70, 80] & 50 & 60\\
    $l_{min}$& - & 20 & 20\\
    \midrule
    Batch size&\{64, 128, 256, 512\}& 128& 128\\
    $lr$&[1e-4, 1e-2]& 8e-3 & 3e-3\\
    $d$&\{10, 20, 30, 40\}& 40 & 30\\
    $d'$&\{4, 6, 8, 10,12\}& 10 & 10\\
    $L$&\{4, 5, 6, 7, 8\}& 5 & 6\\
    $w_{t}$&\{0, 0.25, 0.5, 0.75, 1\}& 1 & 1\\
    $h$&\{1, 2, 3, 4, 5, 6, 7, 8\}& 4 & 6 \\
    \bottomrule
    \end{tabular}
    % }
    \label{tab:hyper}
	%\vspace{-5mm}
\end{table}

\subsubsection{\textbf{Case Study}}
In addition to the quantitative studies, we demonstrate the effectiveness of \textit{IRN} with a real case.
% by studying how movie genres shift progressively along with the influence paths. 
% For movielens dataset, there are $13$ genres after filtering out "Unknown" and each movie can be associated with multiple genres. To observe clearer genre conversion in the recommendation path, we randomly select the single genre movie as objective and select the testing sequences that end with single genre movie. We set the maximum path length to $10$ and visualize the recommendation path by tracing the name and genre of the movies.
We provide a real influence path generated by \textit{IRN} from the Movielens dataset. As is shown in Table \ref{tab:genre_example}, the \textit{Mille bolle blu} with a genre of ``Comedy'' was selected as the objective item while the user's viewing history ends at \textit{Bulletproof} with a genre of ``Action''. In the initial few steps, \textit{IRN} recommended movies in ``Action'', ``Adventure'', and ``Thriller''. After a few swinging attempts between ``Adventure'' and ``Thriller'', the \textit{Space Jam} with genres ``Adventure'', ``Children'', and ``Comedy'' was recommended, followed by \textit{First Kid} with genres ``Children'' and ``Comedy''. The last few movies are classified into ``Comedy''.  From the example, we can observe a smooth genre transition from ``Action'' to ``Comedy''. The results affirm the effectiveness of \textit{IRN} in leading the user towards the objective item smoothly. 

\begin{table}[tb]
\renewcommand{\arraystretch}{1.3}

% 	\setlength{\belowcaptionskip}{-5pt}
% 	\setlength{\abovecaptionskip}{3pt}
    \caption{An Example of Movie Genre Shifting (* refers to the objective item). }
    \centering

    % \resizebox{0.47\textwidth}{!}{
    \begin{tabular}{ll}
    \toprule
    \bf Name & \bf Genre\\
    \midrule
    \multicolumn{2}{l}{\bf The last movie in the viewing history:}\\
    % Arrival, The (1996)&Action, Sci-Fi, Thriller\\
    % Maximum Risk (1996)&Action, Adventure, Thriller\\
    Bulletproof (1996) & Action\\
    \midrule
    \multicolumn{2}{l}{\bf The movies in the influence path:}\\
    Lost World: Jurassic Park (1997)	&		Action, Adventure, Sci-Fi, Thriller\\
    Chain Reaction (1996)	&		Action, Adventure, Thriller\\
    Anaconda (1997)		&	Action, Adventure, Thriller\\
    Broken Arrow (1996)	&		Action, Thriller\\
    Fled (1996)	&		Action, Adventure\\
    Glimmer Man (1996)	&		Action, Thriller\\
    Space Jam (1996)	&		Adventure, Animation, Children,\\ 
                        &       Comedy, Fantasy\\
    First Kid (1996)	&		Children, Comedy\\
    Jack (1996)		&	Comedy, Drama\\
    Michael (1996)	&		Comedy, Romance\\
    \textbf{Mille bolle blu (1993)}*	&		Comedy\\
    \bottomrule
    \end{tabular}
    % }
    \label{tab:genre_example}
% 	\setlength{\belowcaptionskip}{-10pt}
% 	\setlength{\abovecaptionskip}{-2pt}
% 	\vspace{-5pt}
\end{table}

% To provide a global view instead of visualizing one example, we calculate the average stepwise genre information entropy and the genre similarity to the last history item and target. Denote the genre of last history item $i_0$ as $g_0$ and the genre of target item $i_t$ as $g_t$, given a recommended item $i_p$ with genre set $X_p$, we calculate the information entropy $H(i_p)$, similarity to last history item $d_0$, and similarity to target item $d_1$ as follows:
% \begin{equation}
%     \begin{aligned}
%         H(i_p) = & -log(\frac{1}{|X_p|})\\
%         d_0 = &\frac{1(g_0 \in |X_p| )}{|X_p|}\\
%         d_1 = &\frac{1(g_1 \in |X_p| )}{|X_p|}\\
%     \end{aligned}
% \end{equation}
% where $1(g_1 \in |X_p|)$ equals to $1$ if the genre set contains $g_1$ or $0$ otherwise. We average these three values at each step over all the testing sequences and the result is shown in Figure \ref{fig:entropy}. In general, the PRS prefers items with multiple genres in the recommendation path, which is reflected by the high entropy of intermediate items in Figure \ref{fig:entropy}(a). This observation is consistent with the example shown in Table \ref{tab:genre_example} where each intermediate movie has at least two genres. On the other hand, we can observe from Figure \ref{fig:entropy}(b) that as the recommendation path extends, the path items are less similar to $i_0$ and more similar to $i_t$ in terms of genres. Despite the abnormal case at $step=1$, in the first half recommendation path the genres of path items are closer to $i_0$ while in the latter half it is closer to $i_t$. To summarize, the recommendation paths generated by the PRS display reasonable genre conversion patterns, which validates the effectiveness of PRS in persuading the user to accept target item from another angle. 

% \begin{figure}[tb]
% %	\setlength{\abovecaptionskip}{-3pt}
% %	\setlength{\belowcaptionskip}{-10pt}
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{PRS/eps/entropy.png}
% 	\caption{Global Genre Conversion. (a) displays the average genre information entropy at each step over the testing sequences. (b) displays the change of genre similarity versus step. }
% 	\label{fig:entropy}
% \end{figure}

% \textcolor{red}{[May just mention an example and does not discuss the global entropy]}

% \subsubsection{Target Selection}
% In the previous sections, we evaluate and discuss the performance of PRS using randomly selected items. As shown in the Figure \ref{fig:eval_setting}(b), there exist alternative way that separates the testing sequences and remain the tail part of the sequence for comparison. Apart from the previous metrics, we utilize the comparison-based metrics Rouge-L $F_{lcs}$, Genre Distance $d_g$, and Semantic Distance $d_{emb}$ mentioned in Section \ref{subsec:compare} to measure the \textit{influence path} given the \textit{Reference Path}. Notice that since there can exist multiple reasonable paths that lead the user to the target, these metrics are supplementary to evaluate the recommendation path. 

% The results of evaluating the model with given targets are shown in Table \ref{tab:given_result}. The last item in each testing sequence is selected as the target and $d_{gap}$ is the length of remained $p_{true}$ (i.e. there are $d_{gap}$ items between the end of user viewing history and the target item). Larger $d_{gap}$ indicates further interest gap between the initial state of the user and the target. ...
% \begin{table}[tb]
% \resizebox{0.47\textwidth}{!}{
% \begin{tabular}{|l|l||l|l|l|l|l|l|l|}
% 		\hline
% 		Datasets & d_{gap}& Hit@20 &  MRR   & IoI & PPL & F_{lcs}  & $d_{g}$ & $d_{emb}$  \\ \hline \hline

%         \multicolumn{1}{|c|}{}&10&&&&&&&\\\cline{2-9}
%         \multicolumn{1}{|c|}{ Movielens-100k}&20&&&&&&&\\\cline{2-9}
%         \multicolumn{1}{|c|}{}&30&&&&&&&\\\hline
%         \multicolumn{1}{|c|}{}&10&&&&&&&\\\cline{2-9}
%         \multicolumn{1}{|c|}{ Movielens-1m}&20&&&&&&&\\\cline{2-9}
%         \multicolumn{1}{|c|}{}&30&&&&&&&\\\hline
%         \multicolumn{1}{|c|}{}&10&&&&&&&\\\cline{2-9}
%         \multicolumn{1}{|c|}{ lastfm}&20&&&&&&&\\\cline{2-9}
%         \multicolumn{1}{|c|}{}&30&&&&&&&\\\hline
% \end{tabular}}
% \caption{Given Target ($i_t = i_q$) Result}
% \label{tab:given_result}
% \end{table}
% \textcolor{red}{[ZHU: Consider remove the whole section that discusses the target selection]}



 


% \noindent\textcolor{red}{[ZHU: the following contents have not been modified.}
% \subsection{Evaluation of Interest Satisfaction} \label{Interest-Satisfaction}
% As a sequential recommendation system, the basic requirement is that it should be able to profile users' interests and recommend items that are in line with users' interest, and hence users are willing to click these recommended items. Normally this aspect is evaluated by the next-item prediction accuracy when offline dataset is given, a higher accuracy indicates this recommendation system can better profile users' interest and recommend acceptable items to users. 

% \subsubsection{Experiment Setting:} 
% As each item rating is associated with the timestamp, we order each user's rated items by time and get the historical sequence $\mathcal{S}^u$ for each user. Same as previous works, we take the most recent item $\mathcal{S}^u_{|\mathcal{S}^u|}$ for testing, the second most recent one $\mathcal{S}^u_{|\mathcal{S}^u|-1}$ for validation and hyperparameter tuning, and the rest ones for model training. 

% \subsubsection{Evaluation Metrics:} 
% In our paper, we adopts Hit@50 (Hit Rate at position 50) and AUC (Area Under the ROC Curve) as the metrics for recommendation accuracy evaluation. Below are the formulas we used for the metric definition:
% \begin{equation}
% 	Hit@50 = \frac{1}{|\mathcal{U}|} \sum_{u \in \mathcal{U}} \textbf{1}(R_{u,\mathcal{S}^u_{|\mathcal{S}^u|}}\leq50) ,
% \end{equation} 	
% \begin{equation}
% 	AUC = \frac{1}{|\mathcal{U}|} \sum_{u \in \mathcal{U}} \frac{\textbf{1}}{|\mathcal{I}\backslash\mathcal{S}^u|}\sum_{j' \in \mathcal{I}\backslash\mathcal{S}^u} \textbf{1}(R_{u,\mathcal{S}^u_{|\mathcal{S}^u|}} < R_{u,j'}),
% \end{equation} 	
% where $R_{u,i}$ is the predicted rank of item $i$ for user $u$ (a smaller $R_{u,i}$ indicates the item $i$ has a higher chance to be liked by user $u$), and $\textbf{1}(a)$ is an indicator function which returns 1 when argument $a$ is true and 0 otherwise.

% \subsubsection{Evaluation Result:}
% Based on above setting and metrics, we summarize the baseline comparison results in Table~\ref{tab:accuracy_baselines}. From the table, we can observe ISRNet outperforms all baselines with regards to the next-item prediction, which shows its ability to profile users' interests and make recommendations that satisfy their interests. This gives us more confidence for adopting ISRNet in our reward function modelling as ISRNet is capable of providing reliable next-item rankings giving user's existing sequence. On the other hand, we can see DDQN also performs quite well. This demonstrated although DDQN is a 'persuasive' recommendation system, it still respects and satisfy users' existing interests to a high degree. One possible reason why DDQN is not doing as well as ISRNet in next-item prediction could be that the target we choose for DDQN is random and can be far away from user's current interest. As DDQN needs to make an recommendation that also takes how to persuade user to develop interest in the target item into consideration, the predicted recommendations then could be a step forward from the 'ground-truth' item in the offline test data and causes this slight discrepancy between predicted item and offline 'ground-truth' item.  

% \begin{table*}[]
% 	\begin{tabular}{|l|l||l|l|l|l|l|l|l|l|}
% 		\hline
% 		Datasets                                    & Metrics &  Random       &  MC   & TransUp & TransRec & FPMC  & RNN & ISRNet & DDQN \\ \hline \hline
% 			\multicolumn{1}{|c|}{MovieLens} & Hit@50     &  0.029    &  0.257  & 0.259  & 0.267   & 0.202 & 0.312   &  { \textbf{0.341}}   & 0.296 \\ \cline{2-10} 
% 		\multicolumn{1}{|c|}{}                      & AUC    &  0.457    &  0.845  & 0.883  & 0.886   & 0.822 & 0.905   & {\textbf{0.915}}   & 0.896 \\ \cline{1-10} 
% 		\multicolumn{1}{|c|}{goodreads} & Hit@50     &  0.0004    &  0.0546  & 0.0793  & 0.0764   & 0.0684 & 0.0481   &  { \textbf{0.1027}}   & 0.0782 \\ \cline{2-10} 
% 		\multicolumn{1}{|c|}{}                      & AUC    &  0.481    &  0.771  & 0.822 & 0.777   & 0.877 & 0.749   & {\textbf{0.886}}   & 0.826 \\ \cline{1-10} 
% 	\end{tabular}
% 	\caption{Recommendation Accuracy Result}
% 	\label{tab:accuracy_baselines}
% 	%	\setlength{\belowcaptionskip}{-10pt}
% 	\setlength{\abovecaptionskip}{-2pt}
% 	\vspace{-4.5mm}
% \end{table*}



% \subsection{Evaluation of Interest Development}
% Apart from the basic interest prediction and satisfaction, another important task of our persuasive recommendation system is that it should help users gradually develop new interest in a topic or an item through a sequence of recommendations. 

% \subsubsection{Experiment Setting:}
% It's much simpler to evaluate the persuasiveness aspect in an online environment, as DDQN can just make recommendations and receive timely feedbacks from users. With only offline datasets given, we need some special treatment for the evaluation. What we adopt is to take ISRNet as user-simulator which is similar as the technique used in \cite{zhao2017deep}. Based on evaluation results in section \ref{Interest-Satisfaction}, ISRNet has the best ability to profile a user's current interest and predict ranking of the next-item given current sequence. So when ISRNet is provided with a sequence of items representing an user's current interaction history and a target item we want to develop user's interest on, ISRNet can output the ranking of the target item and a higher ranking indicates currently this users has a higher probability to be interested in this item. 

% Similarly, we order each user's rated items by time and get the historical sequence $\mathcal{S}^u$ for each user. In the evaluation of this subsection, we take the first 90\% items as the current sequence $\mathcal{S}^{u,c}$ and the most recent item $\mathcal{S}^u_{|\mathcal{S}^u|}$ as target item. Our recommendation system will recommend an item $\hat{i}$ based on $\mathcal{S}^{u,c}$ and $\mathcal{S}^u_{|\mathcal{S}^u|}$. If the recommended item $\hat{i}$ is accepted by the user, we will append $\hat{i}$ to $\mathcal{S}^{u,c}$, otherwise, we will stop this persuasive recommendation evaluation procedure. In our experiment, if $\hat{i}$ is within user-simulator ISRNet's top-50 ranked items, we will treat $\hat{i}$ as accepted by the user. We limit the maximum length of $\mathcal{S}^{u,c}$ to |$\mathcal{S}^u$| to avoid potential infinity, this limitation also makes the persuasive sequence more realistic as user does reach the target item $\mathcal{S}^u_{|\mathcal{S}^u|}$ with a sequence of length |$\mathcal{S}^u$| in the offline date.

% \subsubsection{Evaluation Metrics:}
% With above evaluation procedure, we name the initial sequence as $\mathcal{S}^{u,i}$ and the final sequence after appending all recommended and accepted items as $\mathcal{S}^{u,f}$. We define below two metrics for persuasiveness comparison:

% \noindent\textbf{Successful Interest Development Rate (SIDR):}
% \begin{equation}
% 	SIDR = \frac{1}{|\mathcal{U}|} \sum_{u \in \mathcal{U}} \textbf{1}(ISRNet(\mathcal{S}^{u,f}, \mathcal{S}^u_{|\mathcal{S}^u|}) > ISRNet(\mathcal{S}^{u,i}, \mathcal{S}^u_{|\mathcal{S}^u|})) ,
% \end{equation} 
% \noindent\textbf{Average Ranking Increase (ARI):}
% \begin{equation}
% 	ARI = \frac{1}{|\mathcal{U}|} \sum_{u \in \mathcal{U}} (ISRNet(\mathcal{S}^{u,f}, \mathcal{S}^u_{|\mathcal{S}^u|}) - ISRNet(\mathcal{S}^{u,i}, \mathcal{S}^u_{|\mathcal{S}^u|})) ,
% \end{equation} 
% where $ISRNet(\mathcal{S}^{u,f}, \mathcal{S}^u_{|\mathcal{S}^u|})$ is $ISRNet$'s ranking of target item $\mathcal{S}^u_{|\mathcal{S}^u|}$ given the final expanded sequence $\mathcal{S}^{u,f}$, while $ISRNet(\mathcal{S}^{u,i}, \mathcal{S}^u_{|\mathcal{S}^u|})$ is its ranking before the persuasive recommendations. A good persuasive recommendation system should have the ability to increase user's interest on target item after conducting a sequence of persuasive recommendations, hence higher SIDR or ARI indicates better performance with regards to the interest development or persuasiveness.

% \subsubsection{Evaluation Result:}
% We compare the persuasiveness performance with the baseline models and summarize the results in Table~\ref{tab:persuasiveness_baselines}. For the Offline column, it uses the ground-truth offline date where $\mathcal{S}^{u,f}$ is defined as the sequence before $\mathcal{S}^u_{|\mathcal{S}^u|}$ in $\mathcal{S}^u$. From this table, we can observe DDQN outperforms all baselines except the ground-truth one. When combining results from Table~\ref{tab:accuracy_baselines} and  Table~\ref{tab:persuasiveness_baselines}, we can draw a clear conclusion that our persuasive recommendation system based on DDQN has the ability to help user develop interest in a target item/topic without sacrificing the click-through-rate and user experience.
 
% \begin{table*}[]
% 	\begin{tabular}{|l|l||l|l|l|l|l|l|l|l|l|}
% 		\hline
% 		Datasets                                    & Metrics &  Offline     & Random    & MC  & TransUp   & TransRec & FPMC & RNN  & ISRNet & DDQN \\ \hline \hline
% 		\multicolumn{1}{|c|}{MovieLens} & SIDR     &  0.607  & 0.465  &  0.501  & 0.506  & 0.474   & 0.517 & 0.523   &  0.502   &  { \textbf{0.566}}  \\ \cline{2-11} 
% 		\multicolumn{1}{|c|}{}                      & ARI    &  42.45  & -35.16  & -9.04  & -14.33  & -19.95  & 1.263 & 4.01   & -2.45   & {\textbf{19.93}} \\ \cline{1-11} 
% 		\multicolumn{1}{|c|}{goodreads} & SIDR     &  0.623  & 0.451 &  0.481  & 0.511  & 0.455   & 0.477 & 0.432   &  0.521   &  { \textbf{0.596}}  \\ \cline{2-11} 
% 		\multicolumn{1}{|c|}{}                      & ARI    &  102.11  & -88.62  &  -21.86 &  17.28  & -55.27  & -42.37 & -84.12   & 25.45   & {\textbf{51.16}} \\ \cline{1-11} 
% 	\end{tabular}
% 	\caption{Interest Development Result}
% 	\label{tab:persuasiveness_baselines}
% 	%	\setlength{\belowcaptionskip}{-10pt}
% 	\setlength{\abovecaptionskip}{-2pt}
% 	\vspace{-4.5mm}
% \end{table*}


==> Influential RS/framework.tex <==

\subsection{Problem Definition}
In sequential recommender systems, user-item interactions are represented as sequences. For a given dataset, we denote the set of all user-item interaction sequences as $S=\{s_1,...,s_{|S|}\}$, which has size $|S|$. Each sequence $s=\{i_1,...,i_{m}\}$ consists of an ordered list of $m$ items. All the items occurring in $S$ constitute the item set $I=\{i_1,...,i_{|I|}\}$ of size $|I|$. 
Let $U$ denote the set of all users, and $S_u$ denote the set of sequences belonging to $u$. We have $S = \mathop{\bigcup}_{u=1}^{|U|} S_u$, where $|U|$ is the number of users. 

The problem of influential recommendation is defined as:
given a user $u$'s viewing history $s_h$ and a selected objective item $i_{t}$, produce a sequence of items, named \textit{influence path} (denoted as $s_p$), which starts from $u$'s original interests and leads $u$ towards $i_{t}$ progressively and smoothly. 
Figure~\ref{fig:eval_setting} illustrates the idea.
An influence path aims to meet two criteria: a path item $i_k$ should expand the user's interests toward the objective $i_t$ and simultaneously satisfy the user's current interests so that the user will not lose patience to the recommendations. The smoothness of the path is also critical since an abrupt recommendation may upset the user. 
Note that $i_t$ can be picked according to the needs of the specific application. 
In this work, we use random $i_t$ to avoid the bias incurred by manual selection. 
\begin{figure}[tb]
% 	\setlength{\abovecaptionskip}{3pt}
% 	\setlength{\belowcaptionskip}{-8pt}
	\centering
	\includegraphics[width=0.47\textwidth]{PRS_problem-eval_setting.png}
	\caption{Illustration of the Influential Recommendation Process. \textit{IRS} recursively recommends a path item $i_k$ until reaching the objective item $i_t$ or exceeding the maximum length allowed. All the path items constitute the influence path $s_p$. }
	\label{fig:eval_setting}
\end{figure}

For simplicity, we assume that the user will passively accept any recommendation, and we employ probability measures to evaluate the user's satisfaction with the influence path. Algorithm \ref{al:ppath} demonstrates the overall workflow of \textit{IRS}. 
The main goal of \textit{IRS} is to learn the recommender function $\mathcal{F}$ that progressively generates the influence path $s_p$ to lead the user towards the objective item and simultaneously satisfy the user's interests. To achieve this goal, we present two baseline solutions adapted from existing \textit{URS} and then our novel influential recommender model.  

\begin{algorithm}
\caption{Generate influence path $s_p$ for user $u$}\label{al:ppath}
\begin{algorithmic}[1]
\STATE \textbf{Input}: Interaction history $s_h$, the objective item $i_{t}$, the maximum path length $M$
\STATE \textbf{Output}: influence path $s_p$
\STATE $s_p$ = [ ]
\WHILE {$|s_p| \leq M$}
  \STATE $i = \mathcal{F}(s_h, i_{t}, s_p)$
  \STATE $s_p = s_p + i$
  \IF {$i$ is $i_t$}
    \STATE break
  \ENDIF
\ENDWHILE
\end{algorithmic}
\label{algo:ppath}
\end{algorithm}

\subsection{Path-finding Algorithms as \textit{IRS}}\label{subsec:pathfinding}
Given the problem setup of \textit{IRS}, it is natural to consider the influence path generation process as a path-finding problem, namely, finding a path between two vertices on a graph that minimizes the cost. 
% By mapping the user's viewing history $s_h$ and the objective item $i_t$ to graph vertices, we convert the \textit{IRS} problem to finding the (shortest) path between two vertices in a graph. 
Since the original dataset is not a graph structure, we build an undirected graph from the user-item interaction sequences following the previous practice \cite{wang2018billion}.
First, we map each item in the training dataset to a graph vertex. 
Then, we assign an edge to two vertices if the corresponding items appear consecutively in an interaction sequence and assign equal weight to each edge. 
For simplicity, we select the last item $i_h$ in the viewing history as the user's recent interest and find a path between $i_h$ and the objective item $i_t$ using a path-finding algorithm such as Dijkstra.
We name this framework as \textit{Pf2Inf}.

Figure \ref{fig:pf_model} illustrates an example of \textit{Pf2Inf}. Given a new interaction history $s_h$ ending at $i_1$ and the objective item $i_{11}$, \textit{Pf2Inf} generates an influence path $s_p = \{i_1, i_6, i_4, i_{11}\}$ based on a shortest path algorithm.


\begin{figure}[tb]
% 	\setlength{\abovecaptionskip}{3pt}
% 	\setlength{\belowcaptionskip}{-10pt}
	\centering
	\includegraphics[width=0.4\textwidth]{PRS_problem-graph.png}
	\caption{An example of \textit{Pf2Inf}. Here we construct an undirected graph from $5$ user-item interaction sequences (one color per user). The arrow indicates the item order within a sequence. }
	\label{fig:pf_model}
\end{figure}

% \subsection{Vector Space Models as \textit{IRS}}
% \label{subsec:vector}
% An intuitive solution for \textit{IRS} is to adapt the existing vector space model for the influential recommendation task. Firstly, we can map users and items to vectors with embedding techniques such as matrix factorization~\cite{koren2009matrix} and neural collaborative filtering~\cite{he2017neural}. Then, a distance-based function $\mathcal{F}$ can be designed to sequentially select an item and add it to the influence path $s_p$ if the item is close to the line connecting the user vector $v_u$ and objective item vector $v_t$ (i.e. the vertical distance is smaller than a given threshold $\theta$). Here, the user vector $v_u$ is computed based on $u$'s viewing history $s_h$. We name this framework as \textit{Vec2Inf}.

% Figure~\ref{fig:vs_model}(a) shows an example of how $s_p$ is generated using \textit{Vec2Inf}. Given $s_h= \{i_1, i_2, i_3, i_4\}$ and an objective item $i_t$, \textit{Vec2Inf} first obtains the user vector $v_u$ and objective item vector $v_t$ and then computes the direct path $p_{u\rightarrow t}$ which starts from $v_u$ and ends at $v_t$. Since $v_5$, $v_6$, and $v_7$ are close to $p_{u\rightarrow t}$, they are selected to constitute the \textit{influence path} $s_p = \{v_5, v_6, v_7\}$, ordered by their distances from $v_u$. 

% \begin{figure}[tb]
% % 	\setlength{\abovecaptionskip}{3pt}
% % 	\setlength{\belowcaptionskip}{-10pt}
% 	\centering
% 	\includegraphics[width=0.47\textwidth]{PRS_problem-vsprs.png}
% 	\caption{An example of \textit{Vec2Inf}. Each item $i_j$ is mapped to a two-dimensional vector. $v_t$ and $v_u$ denote the objective item and user vectors, respectively. The user's viewing history $s_h = \{i_1, i_2, i_3, i_4\}$.}
% 	\label{fig:vs_model}
% \end{figure}

\subsection{Adapting Existing \textit{RS} with Greedy Search}
\label{subsec:rec2pros}

Despite its simple architecture, \textit{Pf2Inf} does not take into account the sequential patterns among items in the user's viewing history.
Neither does it work for sparse, disjoint graphs which are likely to exist in the sparse recommendation dataset. For example, in Figure~\ref{fig:pf_model}, given the interaction history $s_h = \{i_3, i_4, i_{10}\}$, it fails to find a reasonable path to the objective item $i_{12}$ by traversing the graph. 
%Moreover, \textit{Pf2Inf} does not consider the personalizing effect. People respond differently to the influential recommendation. That means, one successful influence path can be rejected by another even though the two persons have similar recent interests.

% Second, it is incapable of handling the case where all items are distant to $p_{u\rightarrow t}$. Figure~\ref{fig:vs_model}(b) shows an example. Since all candidate items (e.g. $v_5$, ..., $v_9$) have large vertical distances to $p_{u\rightarrow t}$, it is hard to generate a reasonable influence path by simply considering items near $p_{u\rightarrow t}$. 
% For example, \textit{Vec2Inf} would have generated the jagged path $s_p = \{v_5, v_7, v_6, v_8, v_9\}$, even though there does exist a better path $s_p = \{v_5, v_7, v_8, v_9\}$.
% it is better to move v6 a little farther from v_u but closer to the straight path to make it easy to see v6 will be selected by vec2pro..  

% It represents the viewing history by averaging all the historical items, where the order information of items (e.g. $v_1$ -> $v_2$ -> $v_3$) is neglected in modelling. On the other hand, 

An alternative is to adapt an existing \textit{RS} to \textit{IRS} using a greedy search strategy. Specifically, we can generate an influence path $s_p$ with the following process: given user $u$'s viewing history $s_h$, an existing \textit{RS} can be used to generate the top-$k$ recommendations $\mathcal{R}_k$, which can then be re-sorted based on their distances to the objective item $i_t$ and the closest item is greedily selected into $s_p$. The recommender repeats the process to generate the whole $s_p$. The distance between two items can be calculated based on their embeddings (e.g. obtained from \textit{item2vec} \cite{he2017neural}). 
With this simple strategy, any existing \textit{RS} can be adapted to generate the influence path, and we name this solution as \textit{Rec2Inf}. 

Depending on the backbone \textit{RS}, the \textit{Rec2Inf} framework can enable a recommender system to model user interests and sequential dependencies among items, and approach the objective item at the same time. However, it still suffers from the following limitations: (1) an item is greedily selected into the influence path in each step. The local optimal selections may not ultimately reach the global optimal influence path. For example, if the objective item $i_t$ deviates from the current user interests significantly and all candidate items in $\mathcal{R}_k$ have large distances from $i_t$, $i_t$ will have little effect in selecting the recommended items, hindering the influence path $s_p$ from reaching $i_t$. (2) The objective item $i_t$ is not involved in the training process, which prevents the \textit{RS} from planning early for reaching the goal of $i_t$ in the entire recommendation process.

% The \textit{Modified Persuasion Recommender System (MPRS)} is adapted based on the \textit{Next-Item Recommender Systems} to conduct persuasion recommendation. Most existing \textit{Next-Item Recommender Systems} consider only the current user interests and generates the recommendation by first obtaining a sorted list of candidate items and recommending the top 1 or top $k$ items to the user. The \textit{MPRS} modifies this process to take the objective item into account as follows. 

%  The recommender $R$ repeats the process to extend the \textit{influence path} with the new viewing history $h = h + i_{top}$ until the objective item $i_t$ is recommended to the user or the path exceeds the maximum allowed length. The generation process can be summarized in Algorithm \ref{al:mprs}:
% \begin{algorithm}
% \caption{Modified Persuasion Recommender System (MPRS)}\label{al:mprs}
% \begin{algorithmic}[1]
% \STATE \textbf{Data}: viewing history $h$, objective item $i_t$, existing recommender $R$, maximum path length $l_{max}$
% \STATE \textbf{Result}: influence path $p$
% \STATE $p = \{\}$
% \IF {$|p|<l_{max}$}
%   \STATE Obtain candidate items set $\mathcal{R}_k = R(h)$
%   \STATE Resort $i_c \in \mathcal{R}_k$ by their distance to $i_t$
%   \STATE Select the top item $i_{top}$ after resorting, update viewing history $h = h + i_{top}$, influence path $p = p + i_{top}$
%   \IF {$i_{top}$ is $i_t$}
%     \STATE break
%   \ENDIF
% \ENDIF 
% \end{algorithmic}
% \end{algorithm}




\subsection{Influential Recommender Network (\textit{IRN})}
\label{subsec:sprs}

% \textit{IRN} captures both the sequential patterns of viewing history and the effects of objective item by utilizing the Transformer decoder~\cite{vaswani2017attention}.

To mitigate the challenges of the \textit{IRS} framework, we propose \textit{Influential Recommender Network} (\textit{IRN}), a neural network model which progressively recommends items to persuade a user to approach the objective. \textit{IRN} can learn the sequential patterns across item sequences, encode the characteristic of the objective item, and consider personalized impressionability at the same time. As shown in Figure~\ref{fig:overall_prsnn}, \textit{IRN} is composed of three components: an embedding layer that vectorizes the input sequence, a stack of $L$ decoder layers, each of which comprises a self-attention layer with personalized masking, and an output layer that projects the hidden states of the decoder into probability distributions over items.

\begin{figure}[tb]
% 	\setlength{\abovecaptionskip}{3pt}
% 	\setlength{\belowcaptionskip}{-8pt}
	\centering
	\includegraphics[width=0.47\textwidth]{PRS_problem-Framework.png}
	\caption{Overall framework of \textit{IRN}. Given a sequence $s = \{i_1, ..., i_m\}$ where the last item is the objective item ($i_t = i_m$), \textit{IRN} first embeds $s$ into vectors. Then it learns the hidden representation of the input sequence with a stack of $L$ decoder layers. The self-attention layers in the decoders incorporate a specially designed \textit{Personalized Impressionability Mask} to cater to users with different acceptance of external influence.}
	\label{fig:overall_prsnn}
\end{figure}

\subsubsection{\textbf{Item Embedding}}
As items are originally represented as discrete tokens, we start by embedding them into dense vectors, which can be processed by deep neural networks. We convert items into both token and position embeddings, which, respectively, represent the context and the position of an item in the sequence. 
Given a sequence of $m$ items~$s = \{i_1, ...i_m\}$, we convert it to a sequence of $d$-dimensional vectors $\mathbf{e}(i_1), ...,\mathbf{e}(i_m)$, with each $\mathbf{e}(i_j)\in R^d$ denoting the embedding for the j-th item, namely,
\begin{equation}
    \mathbf{e}(i_j) = ~TE[i_j] + PE[j]~\mathrm{for}~j = 1, ..., m
\end{equation}
where $TE\in R^{|I|\times d}$ denotes the token embedding matrix and $PE\in R^{m\times d}$ denotes the positional encoding matrix, and "+" refers to addition. 
Inspired by the well-known finding in \textit{NLP} that better initial weights of token embedding can significantly improve the ultimate model performance~\cite{qiu2020pre}, we use pre-trained embedding generated by the \textit{item2vec} model~\cite{barkan2016item2vec}. 

\subsubsection{\textbf{Decoder}}
A Transformer decoder takes the embedding sequence as input and sequentially generates items of the influence path based on the access history and the objective item. 
The decoder maintains a sequence of hidden states $\mathbf{H}= \mathbf{h}_1,...,\mathbf{h}_m$ for the items in the sequence. The hidden state for item $i_j$ is computed based on the items before $i_j$ and the objective $i_t$:
\begin{equation}
    \mathbf{h}_j = \mbox{Dec} (\mathbf{h}_{<j}, \mathbf{h}_t)
\label{equ:dec}
\end{equation}
where $\mathbf{h}_j$ denotes the hidden state of $i_j$. 
The decoder consists of a stack of $L$ self-attention layers with each layer updating the hidden states based on the previous layer. 
\begin{equation}
    \mathbf{H}^{l} = \mbox{Self-Attn}(\mathbf{H}^{l-1})
    \label{equ:dec_wo_u}
\end{equation}
By stacking multiple decoder layers, the model is capable of learning more complicated patterns across the item sequence.
In particular, the first decoder layer takes as input the embedding sequence as the initial hidden states: $\mathbf{H}^0 = \mathbf{e}(i_1), ...,\mathbf{e}(i_m)
$. Here, the self-attention layer performs the layer-wise transformation of the hidden states through the attention mechanism. It takes the hidden states $\mathbf{H}$ as the input for query, key, and value to produce the aggregated value:
\begin{equation}
   \begin{split}
    & \mbox{Self-Attn}(\mathbf{H}) = \mbox{Attention}(\mathbf{H}, \mathbf{H}, \mathbf{H})\\
    & \text{Attention} (\mathbf{Q}, \mathbf{K}, \mathbf{V}) = \text{softmax}(\mathbf{QK}^T/\sqrt{d_k})^T\mathbf{V}
    \end{split}
\end{equation}
where $\mathbf{Q}, \mathbf{K}, \mathbf{V}$ denote the query, key, and value vectors, respectively. Specifically, we use multi-head attention, which is able to attend to information from different representation subspaces at different positions~\cite{li2018multi,sun2019bert4rec, kang2018self}. To enable the decoder to be aware of the objective item, we extend the self-attention layer with a \textit{Personalized Impressionability Mask} (\textit{PIM}). The \textit{PIM} determines (1) which items can be seen by the attention layer, and (2) to what extent the item will be aggregated to produce the hidden states.
We will discuss the two effects of \textit{PIM} in the following sections.

% the multi-head attention, which is able to attend to information from different representation subspaces at different positions~\cite{li2018multi, vaswani2017attention,sun2019bert4rec, lv2019sdm}.  it projects the hidden states $\mathbf{H}$ into $h$ subspaces, and produces the aggregated value by concatenating outputs of paralleled attention functions: 
% \begin{equation}
%   \begin{split}
%     & \mbox{Self-Attn}(\mathbf{H}) = \mbox{Multihead}(\mathbf{H})=[\mbox{head}_1, ..., \mbox{head}_h]\mathbf{W}^O\\
%     & \mbox{head}_a = \mbox{Attention} (\mathbf{H}\mathbf{W}_a^Q, \mathbf{H}\mathbf{W}_a^K, \mathbf{H}\mathbf{W}_a^V)\\
%     & \text{Attention} (\mathbf{Q}, \mathbf{K}, \mathbf{V}) = \text{softmax}(\mathbf{QK}^T/\sqrt{d_k})^T\mathbf{V}
%     \end{split}
% \end{equation}

\begin{figure}[tb]
% 	\setlength{\abovecaptionskip}{3pt}
% 	\setlength{\belowcaptionskip}{-8pt}
	\centering
	\includegraphics[width=0.47\textwidth]{PRS_problem-mask.png}
	\caption{Personalized Impressionability Mask (PIM). $\{i_1,..., i_m\}$ is the input sequence, where the last item $i_m$ is the objective item. (a) displays the standard mask of the decoder. For example, at the second line where the model predicts $i_3$, only $i_1$ and $i_2$ (in blue squares) are perceived by the attention layer while the follow-up items are masked. (b) displays the special mask to reveal the objective, and (c) displays the \textit{PIM} decided by the personalized impressionability factor $r_u$.}
	\label{fig:mask}
% 	\vspace{-5mm}
\end{figure}

\subsubsection{\textbf{Perceiving objective}}
\label{subsubsec:p_attention_mask}
\textit{PIM} is an extension of the standard attention mask in that it enables the decoder to perceive not only previous items but also the objective item. Figures~\ref{fig:mask}(a) and \ref{fig:mask}(b) illustrate the idea. The standard Transformer decoder utilizes a causal (triangular) attention mask to prevent future items from participating in the prediction. Based on the causal attention, \textit{PIM} introduces attention weights to the objective (Figure~\ref{fig:mask}(b)). This enables the attention layer to be aware of the objective item $i_t$ in addition to the preceding items so that it can take in the extra effect of $i_t$ in generating the hidden states. 

Furthermore, we propose a weighted attention mask to reflect the influence of the objective item $i_t$ ($i_t = i_m$). As shown in Figure~\ref{fig:mask}, each item in the input sequence corresponds to a mask weight (i.e. blue square), which will be added to calculate the attention weight inside the decoder. The item with a larger mask weight may contribute more since its corresponding attention weight is larger. Consequently, the item will be regarded as more relevant in generating the output. Let $w_t$ denote the mask weight for the objective item and $w_h$ denote the mask weight for the preceding history. We enforce the model to pay more attention to the objective item by setting $w_t > w_h$. Additionally, by varying the scale of $w_t$, we can control the aggressiveness degree of \textit{IRN} in performing influential recommendations.

\subsubsection{\textbf{Personalized Impressionability Factor}}
Users have personalized curiousness of exploration \cite{zhao2016much}, which may affect their acceptance of external influence. For an impressionable user, \textit{IRN} can be more aggressive and assign more weight to the objective, while for users who have focused interests, \textit{IRN} should be less aggressive in approaching the objective and consider more the user's historical interests. 
We define the \textit{Impressionability} that measures the users' acceptance of persuasion and utilize the \textit{Personalized Impressionability Factor}, denoted by $r_u$, to control the aggressiveness of influential recommendation. $r_u$ is integrated into the mask weight so that the self-attention model can have varying strategies for different users. $r_u$ is computed as:
\begin{equation}
\begin{aligned}
 &\mathbf{e}(u) = ~\mathcal{U}[u] \\
 & r_u = ~\mathbf{W}^U\mathbf{e}(u)
\end{aligned}
\end{equation}
where $\mathbf{e}(u)$ denotes the embedding of $u$ with dimension $d'$, $~\mathcal{U}$ denotes the user embedding matrix, and $\mathbf{W}^U \in \mathbb{R}^{1 \times d'}$ denotes the parameters of the linear transformation. 
The factor $r_u$ is multiplied by the initial attention mask weight for the objective item $w_t$, resulting in the final attention weights (Figure~\ref{fig:mask}(c)). By integrating $r_u$ into the decoder, Equations~\ref{equ:dec} and \ref{equ:dec_wo_u} are extended as:
\begin{equation}
   \begin{split}
    & \mathbf{h}_j = ~ \mbox{Dec}(\mathbf{h}_{<j}, \mathbf{h}_t, r_u)\\
    & \mathbf{H}^{l} = ~ \mbox{Self-Attn}(\mathbf{H}^{l-1}, r_u),~\mathrm{for}~l=1, ...,L
    \end{split}
\end{equation}

\subsubsection{\textbf{Pre-padding Input Sequences}}
The original item sequences can have varying lengths. Therefore, to accommodate the \textit{PIM}, we apply pre-padding on the input sequence instead of the widely used post-padding scheme~\cite{dwarampudi2019effects}. For example, if the maximum sequence length is 5, then the pre-padded sequence for $\{i_1, i_2, i_3\}$ is $\{PAD, PAD, i_1, i_2, i_3\}$, while the post-padded sequence is $\{i_1, i_2, i_3,\allowbreak PAD, PAD\}$, where $PAD$ is the padding token. Pre-padding allows the objective item to stay at a fixed position (i.e., the last item in the sequence) whereas post-padding has different positions for the objective item depending on the sequence length. The fixed position of the objective item avoids extra noise brought to the model due to the variable-length input sequences in position encoding and accelerates the computation~\cite{li2021easy}.
% The objective item is always placed at the fixed position (the end of the input sequence) regardless of the length of the actual sequence, avoiding the extra noise brought to the model due to the variant-length of the the input sequence. 
% which facilitates the use of \textit{Personalized Attention Mask}. (2) The objective item has fixed positional encoding and the position representation of the input is more accurate \cite{li2021easy}. For the same example, it will be converted to $\{i_1, i_2, PAD, PAD, i_3\}$ if post-padding is applied. The original sequence is partitioned, and consequently the position information of the actual sequence may not be well represented by the positional encoding. 

\subsubsection{\textbf{Output Probability}}
Finally, we project the decoder output $\mathbf{H}^L = \{\mathbf{h}_1^L, ..., \mathbf{h}_m^L\}$ to the item space with a linear layer and generate the output probability using the softmax function. Formally, the probability distribution for generating the $j$-th item can be computed as:
\begin{equation}
    \begin{aligned}
    p(i_j|i_{<j}, i_t, u) = \mbox{softmax}(\mathbf{W}^p \mathbf{h}_{j-1}^L)
    \end{aligned}
\end{equation}
where $W^p \in \mathbb{R}^{|I| \times d}$ is the projection matrix.
\textit{IRN} recommends an influence path by generating items one by one according to the probability distribution $p(i_j|i_{<j}, i_t, u)$ at each step. 

\subsubsection{\textbf{Objective Function}}
Given a sequence of items $s = \{i_1, ..., \allowbreak i_m\}$ for user $u$ ($s \in S_u$), where the last item is selected as the objective item ($i_t = i_m$). Assuming that $u$'s interests start at $i_1$, the actual path from $i_1$ to $i_m$ should have maximized probability, which is equivalent to minimizing the conditional perplexity:
\begin{equation}
\begin{aligned}
    \mathrm{PPL}(i_1,...,i_m|i_t, u) =&~ P(i_1,...,i_m|i_t, u)^{-\frac{1}{m}}\\
    =&~\bigg(\prod_{j=1}^m P(i_j|i_{<j}, i_t, u)\bigg)^{-\frac{1}{m}}
    \label{equ:cond_pp}
\end{aligned}
\end{equation}
Apart from items preceding $i_j$ in the sequence, the conditional probability of $i_j$ considers both the objective item $i_t$ and the personalization of $u$. 
To avoid numerical underflow, we minimize its logarithmic form instead, which is equivalent to minimizing the cross-entropy loss function:
\begin{equation}
    \mathcal{L} = \frac{1}{|S|}\sum_{u\in U}\sum_{s\in S_u} \bigg(-\frac{1}{m}\sum_{j=1}^m \log P(i_j|i_{<j}, i_t, u)\bigg)
\end{equation}
where $S = \mathop{\bigcup}_{u=1}^{|U|} S_u$. It is worth noting that each sequence $s=\{i_1,...,\allowbreak i_m\}$ belongs to one user and one user may have multiple sequences. 

% The persuasiveness recommender system (PRS) has the two following properties compared with most existing recommender system. Firstly, apart from the immediate reward of fitting the user interests, the recommended item yields long-term reward in shifting the user interests towards the objective item. Secondly, given the dynamic property of item space (e.g. hot videos), conducting online updates rather than expansive offline updates is more preferable in the scenario. Therefore, we adopt the reinforcement learning method, Double Deep Q-learning Network (DDQN) to model the persuasiveness recommender system. 

% In the remaining sections, we will explain the recommender system in the following order: ISRNet and NPNet, reward and state transition design, DDQN components, and overall algorithm.

% \subsection{Item Sequence Representation Network and Next-item Prediction Network} \label{subsub:models}

% We propose Item Sequence Representation Network (ISRNet) to represent the user state sequence~$s_t$ and Next-item Prediction Network (NPNet) to estimate the conditional probability~$p(tar|s_t)$, respectively. The ISRNet is built on the basis of Transformer, a state-of-the-art sequence representation model. As shown in Figure~\ref{fig:isrnet}, the ISRNet takes a sequence of items as input. All items are converted into item embeddings, which are then fed to a transformer encoder (i.e., a stack of self-attention layers) in order to compute the sequence representation~$s_t$. The NPNet, as shown in Figure~\ref{fig:tpn}, is an fully connected neural network classifier based on the ISRNet. Given the user status sequence, it first represents the sequence using the ISRNet. Then, an extra feed-forward layer with softmax is employed to classify the next item. The NPNet finally outputs the probability distribution $p(tar|s_t)$ at each step. We optimize the model by minimizing the cross entropy loss with respect to these predictions:
% \begin{equation}\label{eq:loss1}
%  L1 = -\frac{1}{T-1} \sum_{t=1}^{T-1} \mathrm{log}~p(i_{t+1}|i_1,...,i_t) 
% \end{equation}
% The ISRNet and NPNet are trained jointly with backpropagation as shown in Algorithm~\ref{alg:tpn}. 

% \subsection{Reward and State Transition}
% \label{subsub:IPRW}

% Under the setting of our framework, the recommended item will receive an immediate reward measuring the current user preference and a long-term reward measuring the interests shifting effect towards the objective item. Therefore, we model the total reward at timestamp $t$ as Equation \ref{equ:reward}.

% \begin{align}
% \label{equ:r1}
% r_1(s_{t},a_{t}) &= pref_u(s_{t},a_{t}) = p(a_{t}|s_{t})\\
% \label{equ:r2}
% r_2(a_t, s_{t},s_{t+1}, a_{tar}) &= p(a_{tar}|s_{t+1})-p(a_{tar}|s_t)\\
% \label{equ:reward}
% r(a_t|s_t, \text{tar}) &=  r_1  +  \textbf{1}(r_1 \geq \lambda_b) \cdot r_2
% \end{align}

% where $s_t$ denotes user's current status (i.e. representation of users' historical interaction sequence), $s_{t+1}$ denotes the users' next status (i.e. representation after appending the recommended item to users' interaction sequence), $a_t$ denotes the recommended item, $a_{tar}$ denotes the objective item. $r_1$ and $r_2$ measure the immediate and long-term rewards respectively. Notice that in online application, the immediate reward $r_1$ can be obtained from the user feedback directly, while in the offline setting it is calculated using approximation, we adopt \textbf{NPNet} in this paper.

% As discussed before, we utilizes the transformer technique (\textbf{ISRNet}) to learn the embedding of user's historical interaction sequence. Considering the state transition, if the recommended item is disfavored by the user, it will be declined regardless of its long-term reward and the user state will remain unchanged. Formally, we define the states and transition process of for the DDQN model as below:

% \begin{itemize}
%     \item \textbf{State} $s$: Given an chronological item sequence $S_u=\{i_1, i_2, ..., i_{k}\}$ of variable length $k$ that the user has given positive feedback, the state $s$ is calculated by $s = ISRNet(S_u)$.
%     \item \textbf{Transition} from $s_t$ to $s_{t+1}$: When the recommender system recommends an item $a_t $to a user with current state $s_t$, he/she may give positive or negative feedback. If positive feedback is given, the item sequence is updated to $S_u'=\{i_2, i_3, ..., i_{k}, a_t\}$ and the new state $s_{t+1} = ISRNet(S_u')$. Otherwise, $s_{t+1} = s_{t}$.
% \end{itemize}

% In the offline setting, we approximate the user feedback using several schemes. Firstly, the next-item prediction network (\textbf{NPNet}) built on the ISRNet can be used to predict the probability, $p$ ,that the user is interested in the recommendation item $a_t$ given user state $s_t$. Then we can discrete this probability values as the user feedback, e.g., $\textbf{1}(p \geq \lambda_b)$.

% In general, the environment under the offline setting is shown in Algorithm~\ref{al:env}. Firstly, we calculate the immediate reward of a recommendation using approximation (line 1). According to the immediate reward, state transition is conducted (line 2) and we calculate the potential long-term reward. Finally, we derive the overall reward of a recommendation.

% \vspace*{-0.1in}
% \begin{algorithm}[H]
% 	\caption{Environment in offline training}
% 	\newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}
% 	\begin{algorithmic}[1]
% 		\STATE Calculate the immediate reward of the item: 
% 		\begin{equation}\nonumber
% 		    r_1 = F_1\big(NPN(a_{tar}|s_{t})\big)
% 		\end{equation}
% 		\STATE Conduct state transition as follows:
% 		\begin{equation}\nonumber
% 		s_{t+1}=\left\{
%             \begin{array}{rcl}
%             ISRNet(\{i_1,i_2,...,i_k,a_t\})       &      & r_1>\lambda_b\\
%             s_t   &      & otherwise\\
%             \end{array} \right.
% 		\end{equation}
% 		\STATE Calculate the long-term persuasive effect of the item: 
% 		\begin{equation}\nonumber
% 		    r_2 = NPN(a_{tar}|s_{t+1})- NPN(a_{tar}|s_{t})
% 		\end{equation}
% 		\STATE Generate the reward of the recommendation: $r_t = r_1+ \textbf{1}(r_1 \geq \lambda_b) \cdot r_2$
% 	\end{algorithmic}
% 	\label{al:env}
% \end{algorithm}

% \subsection{Double Deep Q-learning Agent}
% \label{subsub:IPRW}

% The general idea of our DDQN-based PRS is that the DDQN agent will compute the Q-value for each item given the current state $s$ and objective item $a_{tar}$, it then selects the item with the highest value as the recommendation $a_t$. Upon receiving the recommendation, the user will give feedback and transit to next state if he/she rates the item positively. Once an item is recommended and accepted, it will be removed from the item space in that round of persuasive recommendation in case of repeated recommendation. Finally, if the agent learns from the state that the user's interests have reached significant level, the agent will select the objective item $a_{tar}$ as the recommendation and the round of persuasive recommendation ends with a terminated stage.

% Double DQN utilizes two identical Deep Q-learning network with one learning in the experience replay and another one calculating the Q-value of an action. By this means, the action selection process is decoupled from the generation of Q-value, which reduces the overestimate at the beginning of the training. The second neural network is updated every $C$ step by copying the first neural network.

% When the agent observes the current state $s_t$, it uses the first neural network $\mathcal{Q}$ to generate the recommendation $a_t$ by finding the item with maximum Q-value. In case of local optimality, randomness is added to the action and it will be descending by number of iterations. 

% \begin{equation}
%     a_t=\left\{
%             \begin{array}{rcl}
%             a_{random} && with~probability~\epsilon\cr
%             \mathop{\arg\max}\limits_{a} \mathcal{Q}(s_t, a)   && otherwise\cr
%             \end{array}\right. 
% \end{equation}

% where $a_{random}$ is a random item in the item space, $\epsilon$ is the probability to select a random item, and $s_t$ is the current state. After receiving the recommendation, the environment will pass reward $r_t$ and next state $s_{t+1}$ to the agent, and the agent will store the transition batch $(s_t, a_t, r_t, s_{t+1})$ in the replay memory.

% In training of model through the experience replay, we randomly sample the transition batch from the replay memory and updating the model by computing the one-step TD error. The Q-value $y_i$ of the action will be calculated using the second neural network as follows:

% \begin{equation}
%     y_i=\left\{
%             \begin{array}{rcl}
%             r_i && if~terminated\cr
%             r_i + \gamma\mathcal{Q}'(s_i,a_i)&& otherwise\cr
%             \end{array}\right. 
% \end{equation}

% Notice that $a_i = \mathop{\arg\max}\limits_{a} \mathcal{Q}(s_i, a)$ is previously selected by the first neural network. Then the model will update the parameters through minimizing the mean square error $\frac1 m \sum^{m}_{i=1} \big(y_i - \mathcal{Q}(s_i,a_i)\big)^2$. In practice, the training process of DDQN is shown in Algorithm \ref{al:ddqn}.

% \vspace*{-0.1in}
% \begin{algorithm}[H]
%     \caption{Training of Double Deep Q-learning (DDQN)}
%     \newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}
%     \begin{algorithmic}[1]
%         %\REQUIRE Critic network $Q(s,a|\theta^Q)$, actor network $\mu(s|\theta^\mu)$, objective network %$Q'(s,a|\theta^{Q'})$ and $\mu'(s|\theta^{\mu'})$
%         \STATE Random initialize action-value function  $\mathcal{Q}(s,a|\theta)$ and objective action-value function $\hat{\mathcal{Q}}(s,a|\hat{\theta})$ with weights $\theta$ and $\hat{\theta}$;
%         \STATE Initialize replay buffer $R$;
%         \FOR{episode = 1, $M$}
%         \STATE Initialize the objective item $a_{tar}$.
%         \STATE Random choose a user sequence $S$ and obtain initial state $s_1$ by feeding it to the item sequence representation network and concatenating with the objective item embedding. 
%         \FOR{t = 1, $T$}
%         \STATE Select a random action $a_t$ with probability $\epsilon$, otherwise select $a_t = argmax_a\mathcal{Q}(s,a|\theta)$
%         \STATE Execute action $a_t$ and receive reward $r_t$ and next state $s_{t+1}$ from the environment. 
%         \STATE Store transition $(s_t,a_t,r_t,s_{t+1})$ in $R$
%         \STATE Sample a random minibatch $(s_i,a_i,r_i,s_{i+1})$ of $m$ transitions from $R$
%         \STATE Set $y_i=\left\{
%             \begin{array}{rcl}
%             r_i && if~terminated\cr
%             r_i+\gamma\hat{\mathcal{Q}}(s_i,a_i|\hat{\theta}) && otherwise\cr
%             \end{array}\right. $
%         \STATE Perform a gradient descent step on $(y_i-\mathcal{Q}(s_i,a_i|\theta))^2$ with respect to the network parameters $\theta$
%         \STATE Set $\hat{\mathcal{Q}}=\mathcal{Q}$ every $C$ steps
%         \ENDFOR
%         \ENDFOR
%     \end{algorithmic}
%     \label{al:ddqn}
% \end{algorithm}

% \iffalse
% In the actor component, the actor will generate an action vector $v_a$ according to the current state $s_t$. Then according to the action vector, we can calculate the score of each item in the item space with size $\mathcal{D}$ as follows:

% \begin{equation}
%     \label{equ: action}
%     score_i = v_a \cdot v_i~ for~ i = 1, 2, ..., \mathcal{D}
% \end{equation}

% where $v_i$ is the embedded vector of the $i^th$ item in the item space. The item with the highest score will be selected as the recommendation item and it will be forwarded to the user, who will rate the item in return. In the setting of offline training, we use the aforementioned total reward (Equation 5) to model the user feedback and long-term reward. Once the item is selected as the recommendation item, it will be removed from the item space in case of repeated recommendation. 

% The critic component $\mathcal{Q}(s_t, a_t)$ is designed to measure the effectiveness of the recommendation $a_t$ given the user state $s_t$. After obtaining $\mathcal{Q}(s_t,a_t)$, the actor updates its parameters accordingly in a direction of improving its recommendation in the following iterations. More formally, the Q-value function is calculated by:

% \begin{equation}
%     \label{equ: Q-value}
%     \mathcal{Q}(s_t,a_t)=\mathbb{E}_{s_{t+1}}[r_t + \gamma\mathcal{Q}(s_{t+1},a_{t+1}|s_t,a_t)]
% \end{equation}

% where $\mathcal{Q}(s_t,a_t)$ is the expected return based on $s_t$ and $a_t$. However, due to the large item space and insufficient information about each state and action pair, it is computational inefficient and unrealistic to calculate the above function. Instead, we can approximate the Q-value function as follows:

% \begin{equation}
%     \label{equ: Approx Q-value}
%     \mathcal{Q}(s_t,a_t) \approx \mathcal{Q}(s_t,a_t|\theta^\mathcal{Q})
% \end{equation}

% Since the Q-value function displays highly nonlinear property, the neural network is used as the function approximator and it is trained by minimizing the loss function: 

% \begin{equation}
%     \label{equ: Loss function}
%     L=\mathbb{E}_{s_i, a_i, r_i, s_{i+1}}[(y_i-\mathcal{Q}(s_i,a_i|\theta^\mathcal{Q}))^2]
% \end{equation}

% where $y_i = r_i+\gamma\mathcal{Q}'(s_{i+1},\mathcal{A}'(s_{i+1}|\theta^{\mathcal{A}'})|\theta^{\mathcal{Q}'})$ is the computed value in this iteration, and parameters $\theta^{\mathcal{A}'}$, $\theta^{\mathcal{Q}'}$ are obtained from the previous iteration. For the actor component, we update its parameters using the policy gradient as below:

% \begin{equation}
%     \label{equ: actor gradient}
%     \nabla_{\theta^{\mathcal{A}}}J\approx \mathbb{E}_{s_i, a_i, r_i, s_{i+1}}[\nabla_a\mathcal{Q}(s,a|\theta^\mathcal{Q})|_{s=s_i, a=\mathcal{A}(s_i)}\nabla_{\theta^{\mathcal{A}}}\mathcal{A}(s|\theta^\mathcal{A})|s_i]
% \end{equation}

% where $\theta^\mathcal{Q}$ and $\theta^{\mathcal{A}}$ are the parameters for critic network $\mathcal{Q}(s,a|\theta^\mathcal{Q})$ and actor network $\mathcal{A}(s|\theta^\mathcal{A})$ respectively. 

% In practice, the training procedure of the DDPG framework is shown in the Algorithm~\ref{al:ddpg}. In each episode, we first randomly initialize the starting state $s_1$ and the exploration noise and select the objective item (line 5, 6). Then in each iteration step, the actor component generates the recommendation item according to the current state (line 8). The environment will give feedback on the recommendation and state transition is conducted (line 9). Then the recommender will store the transition batch ($s_t, a_t, r_t, s_{t+1}$) in the memory buffer (line 10). Later, we sample a random minibatch from the memory buffer to conduct the parameter update of critic network $\mathcal{Q}(s,a|\theta^\mathcal{Q})$ and actor network $\mathcal{A}(s|\theta^\mathcal{A})$ according to the Equation 9 and Equation 10 (line 20-23). Finally, the objective network $\mathcal{Q}'(s,a|\theta^\mathcal{Q}')$ and $\mathcal{A}'(s|\theta^\mathcal{A}')$ is updated accordingly (line 24). Notice that in next iteration, the current state becomes $s_{t+1}$.

% \fi



% % list of TBD
% % state definition (positive or viewed)
% % state transition (fixed length)
% % action selection problem (one hot? item embedding)
% % the action embedding/vector used in the Q-value function 
% % modificatin to the policy gradient
% \subsection{Overall Framework}
% In summary, the overall algorithm of the persuasive recommender system is shown in Algorithm~\ref{al:overall}. In stage 1, we follow Algorithm \ref{alg:tpn} to jointly train the item sequence representation network (ISRNet), used to derive state embedding vector according to the user viewing history $S_u=\{i_2, i_3, ..., i_{k}\}$, and the next-item prediction network (NPNet), used to calculate the probability of user being interested in the item $a$ given the current state $s_t$. In stage 2, the environment is initialized and finally in stage 3, the double Deep Q-learning network (DDQN) is trained following Algorithm \ref{al:ddqn} and used to generate recommendation.

% \vspace*{-0.1in}
% \begin{algorithm}[H]
% 	\caption{Persuasive Recommender Framework}
% 	\newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}
% 	\begin{algorithmic}[1]
% 	    \STATE \textbf{Stage 1: Trainthe ISRNet and NPNet}
% 	    \STATE \textbf{Stage 2: Initialize the Environment}
% 		\STATE \textbf{Stage 3: Train the DDQN}
% 	\end{algorithmic}
% 	\label{al:overall}
% \end{algorithm}




% \iffalse 


% \vspace*{-0.1in}
% \begin{algorithm}[H]
%     \caption{Training of Deep Deterministic Policy Gradient (DDPG) recommender}
%     \newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}
%     \begin{algorithmic}[1]
%         %\REQUIRE Critic network $Q(s,a|\theta^Q)$, actor network $\mu(s|\theta^\mu)$, objective network %$Q'(s,a|\theta^{Q'})$ and $\mu'(s|\theta^{\mu'})$
%         \ENSURE Next-item prediction network and item sequence representation network is trained;
%         \STATE Random initialize critic network $\mathcal{Q}(s,a|\theta^\mathcal{Q})$ and actor network $\mathcal{A}(s|\theta^\mathcal{A})$ with weights $\theta^\mathcal{Q}$ and $\theta^\mathcal{A}$;
%         \STATE Initialize objective network $\mathcal{Q}'$ and $\mathcal{A}'$ with weights $\theta^{\mathcal{Q}'}=\theta^\mathcal{Q}$,  $\theta^{\mathcal{A}'}=\theta^\mathcal{A}$;
%         \STATE Initialize replay buffer $R$;
%         \FOR{episode = 1, $M$}
%         \STATE Initialize a random process $N$ for action exploration
%         \STATE Random choose a user sequence $S$ and obtain initial state $s_1$ using item sequence representation network. Initialize the objective item $a_{tar}$
%         \FOR{t = 1, $T$}
%         \STATE Select action $a_t=\mathcal{A}(s_t|\theta^\mathcal{A})+N_t$ according to the current policy and exploration noise
%         \STATE Execute action $a_t$ and receive reward $r_t$ and next state $s_{t+1}$ from the environment. 
%         \STATE Store transition $(s_t,a_t,r_t,s_{t+1})$ in $R$
%         \STATE Sample a random minibatch of $m$ transitions from $R$
%         \STATE Set $y_i = r_i+\gamma*\mathcal{Q}'(s_{i+1},\mathcal{A}'(s_{i+1}|\theta^{\mathcal{A}'})|\theta^{\mathcal{Q}'})$
%         \STATE Update critic by minimizing the loss: $L=\frac{1}{N}\sum_{i}(y_i-\mathcal{Q}(s_i,a_i|\theta^\mathcal{Q}))^2$
%         \STATE Update the actor policy using the sampled policy gradient
%         \STATE Update the objective networks:
%         \begin{equation}\nonumber
%         \begin{split}
%         \theta^{\mathcal{Q}'}=\tau\theta^\mathcal{Q}+(1-\tau)\theta^{\mathcal{Q}'}\\
%             \theta^{\mathcal{A}'}=\tau\theta^\mathcal{A}+(1-\tau)\theta^{\mathcal{A}'}
%         \end{split}
%         \end{equation}
%         \ENDFOR
%         \ENDFOR
%     \end{algorithmic}
%     \label{al:ddpg}
% \end{algorithm}



% \vspace*{-0.1in}
% \begin{algorithm}[H]
%     \caption{Generate experience buffer manually}
%     \newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}
%     \begin{algorithmic}[1]
%         \STATE Initialize replay buffer $R$;
%         \FOR{each user sequence $S_i$}
%         \FOR{t = 1, $N$}
%         \STATE Select a random position $k$, generate sub-sequence $\{i_1, i_2, ..., i_k\}$. Select a random objective item $a_{tar} = i_j$, where $j>k+1$. Obtain state $s$ by concatenating the sub-sequence embedding and objective item embedding.
%         \STATE Obtain positive action $a_{pos}=i_{k+1}$ and set its reward $r_{pos} = 1$. Obtain next state $s_{next}$ from the sub-sequence $\{i_1, i_2, ...,i_k, i_{k+1}\}$ and $a_{tar}$.
%         \STATE Store transition batch $(s, a_{pos}, s_{next}, r_{pos})$ in the buffer.
%         \STATE Obtain negative action $a_{neg}$ by selecting a random item outside the user sequence and set its reward $r_{neg} = -1$. Obtain next state $s_{next} = s$.
%         \STATE Store transition batch $(s, a_{neg}, s_{next}, r_{neg})$ in the buffer.
%         \ENDFOR
%         \ENDFOR
%     \end{algorithmic}
%     \label{al:gm}
% \end{algorithm}

% \subsection{Overall Algorithm}
% \label{subsub:IPRW}
% \fi


% \begin{figure}
% %	\setlength{\abovecaptionskip}{-3pt}
% %	\setlength{\belowcaptionskip}{-10pt}
% 	\flushleft
% 	\includegraphics[scale=0.35]{ddqn.pdf}
% 	\caption{Illustration of Persuasive RS Framework}
% 	\label{fig:framework}
% \end{figure}



==> Influential RS/intro.tex <==
\textit{Recommender system} (\textit{RS}) has created huge business values for applications such as e-commerce, advertising, and streaming media. Traditional \textit{RS} tries to learn users' internal interests from their historical user-item interactions and recommend items judged to be relevant to the users' interests. 
Despite the recent advancements of \textit{RS} in modeling the users' long/short-term interests, most existing works on \textit{RS}s are passive in that their recommendations are driven by users' historical interests. If the user does not respond to a recommendation positively, these \textit{RS}s would try to please the user by selecting another item that better fits the user's interest. In other words, they model the users' interests and fit their recommendations to the user's internal interests instead of proactively developing their external interests. We refer to this \textit{RS} approach as \textit{User-oriented Recommender System} (\textit{URS}).

For many commercial applications, a business may want its recommendation system to be able to \textit{influence} users to like an objective item that they originally may not be interested in by expanding the users' current interests. This allows a business to develop effective branding and marketing strategies by enticing users to pay attention to some promotional or new-arrival items. A \textit{URS} would not be able to achieve this goal since it only displays items within the users' interests. On the other hand, a straightforward advertisement placement system will simply display the objective items to the users, amounting to hard-selling the items to the users. Neither is desirable from a business or user point of view.
In this paper, we propose a new \textit{RS} paradigm named \textit{Influential Recommender System} (\textit{IRS}). \textit{IRS} aims to influence a user $u$'s interest towards a given objective item $i_t$ by recommending a sequential list of items (called \textit{influence path}), which not only follows $u$'s historical interests but also progressively broadens $u$'s interests towards the objective $i_t$. 
% May further explain the use of term "influencing"

\begin{figure}[tb]
    \flushleft
	\includegraphics[width=0.5\textwidth]{intro-new-movie.pdf}
	\caption{Illustration of Influential Recommender System.}
	\label{fig:example}
% 	\vspace{-5pt}
\end{figure}

Figure~\ref{fig:example} illustrates the idea of \textit{IRS} in a movie recommendation scenario. Solid arrows indicate users' viewing histories (one color per user), which reflect the users' chronological behavioral sequences of movie watching. These sequences reflect not only the users' interests profile but also the movies’ sequential dependencies. In the example, Bob is interested in fantasy movies, with a watch history of \textit{The Matrix} $\rightarrow$ \textit{The Abyss} $\rightarrow$ \textit{The Terminator} $\rightarrow$ \textit{Avatar} $\rightarrow$ \textit{Source Code},
% $The\;Matrix \rightarrow The\;Abyss \rightarrow The\;Terminator \rightarrow Avatar \rightarrow Source\;Code$, 
in which all movies are of the fantasy genre. Similarly, Tom is a fan of director James Cameron, and Jenny likes romance movies.

Assume that the goal of \textit{IRS} is to influence Eric to watch the objective movie \textit{The Notebook}, a classic romance movie. From Eric's watch history, \textit{Inception} $\rightarrow$ \textit{The Matrix}, it is fair to infer that Eric has a high chance of accepting fantasy movies, but how can \textit{IRS} lead him to watch the romance movie \textit{The Notebook}?

We notice that Eric and Tom both watched \textit{The Matrix}. Thus, there is a good chance for Eric to accept Tom's behavioral sequence, i.e., 
\textit{The Abyss} $\rightarrow$ \textit{The Terminator} $\rightarrow$ \textit{Avatar}.
After Eric accepts \textit{Avatar}, a romance movie directed by Cameron, we are more confident to say that Eric has developed a certain level of interest in Cameron and the romance genre. Taking one step forward, we can recommend \textit{Titanic}, another classic romance movie directed by Cameron, to Eric. If Eric accepts it, his interest in romance movies is further strengthened. Following Jenny's sequence, recommending \textit{The Notebook} as the next movie for Eric becomes natural and persuasive. This potential recommendation sequence (called \textit{influence path}) is indicated by the green dash arrows. This example illustrates the goal of \textit{IRS}, that is, the progressive expansion of a user's interest towards the objective item along an enticing, smooth influence path learned from the large historical user data.



There are key differences between \textit{URS} and \textit{IRS}. For \textit{URS}, users play the central role, and \textit{URS} aims to adapt to the users' historical interests, while for \textit{IRS}, the platform takes the proactive role to leading the users to like the preset objective items by progressively recommending a carefully selected sequence of items. Filling the gap from \textit{URS} to \textit{IRS} presents several challenges. 
First, the influence path should (i) not deviate too much from the user’s historical interest in order to maintain the user’s trust and satisfaction with the system and (ii) progressively recommend items related to the objective item so that the user’s interest in the objective item can be developed and the transition from the user's interest towards the objective item is gradual and smooth. 
Second, user-item interactions have sequential patterns, i.e., the next item/action depends more on items/actions the user engaged in recently \cite{tang2018personalized}. Thus, the generation of an influence path must align with the sequential dependencies among the items. 
Third, a user's preference for external influence is personal. That is, some users may be extrovert, i.e., they favor exploration and thus can be easily affected by external influences, but some may favor staying in their comfort zone and are difficult to be persuaded to accept new interests. For the former, influence paths could be more aggressive, i.e., they can deviate more from the users' existing interests to reach the objective item in fewer steps; for the latter, the reverse should be taken. We introduce the notion of \textit{Impressionability} to account for the users' different preferences of external influence.


To meet these challenges, we propose \textit{Influential Recommender Network} (\textit{IRN}), which is adapted based on the widely used \textit{Transformer} model \cite{vaswani2017attention} in natural language processing (\textit{NLP}).
Both the user-item interaction sequences and \textit{NLP} sentences have a sequential structure, and the dependencies among items/words exist not only in adjacent items/words but also among distant items/words, which can be well captured by the multi-head attention mechanism. 
Furthermore, to accommodate the influence of the objective item and to personalize the generation of the influence path for individual users with different degrees of impressionability, we design a new masking scheme termed \textit{Personalized Impressionability Mask} (\textit{PIM}) that incorporates user embedding into the calculation of item attention weights. 

To the best of our knowledge, we are the first to propose influential recommendations. Consequently, there are no standard performance metrics or similar approaches to serve as baselines for performance evaluation. 
To overcome these problems, we design new performance metrics that can be used to measure whether the proposed \textit{IRS} frameworks can lead the user to the objective item while satisfying the user's current interest. As explained in Section~\ref{sec:experiment}, we need to determine how much a user is interested in an unseen item, which cannot be obtained from offline datasets. Thus, we propose to use an \textit{Evaluator} to simulate the reaction of a user to an unseen item. 
% We compare our approach with seven traditional recommender systems such as  \textit{TransRec}~\cite{he2017translation} and \textit{Caser}~\cite{tang2018personalized}. 

%To obtain a fair and comprehensive evaluation, we adapt traditional \textit{URS}s (e.g. \textit{TransRec}~\cite{he2017translation} and \textit{Caser}~\cite{tang2018personalized}) to perform \textit{IRS} functions using two alternative frameworks. 
%Then, we compare our approach with seven adapted baseline models.
%Further, we use offline recommendation datasets that have the properties suitable for evaluating \textit{IRS}.
% analyze the influence paths generated by different approaches in conducting smooth and successful influential recommendation. 
% we present a detailed analysis of the influence paths generated by different approaches and demonstrate a real influential recommendation example to illustrate the idea of \textit{IRS}
%Experimental results show that \textit{IRN} significantly outperforms baseline recommenders in terms of success rate and smoothness. Case study has demonstrated its capability of influencing user's interest.


The contribution of this paper is multi-fold:
\begin{enumerate}
\item We propose a new paradigm of recommendation named \textit{Influential Recommender System} (\textit{IRS}), which proactively leads the user towards a given objective item instead of passively adapting the recommendations to the user’s historical interests. To the best of our knowledge, \textit{IRS} is the first to infuse proactivity and influence to \textit{RS}s.

\item We design \textit{Influential Recommender Network} (\textit{IRN}), a Transformer-based model to encode the items' sequential dependencies. In order to model the user's personalized preference of external influence, we extend Transformer by adding user embedding to the attention mechanism.

% \item We implement the SPRS by adapting the transformer model. The trained network is capable of generating a recommendation path given the viewing history of the user and the target item. 

\item We design several performance metrics and offline experiments specifically for evaluating \textit{IRS}. Experimental results show that our proposed \textit{IRN} significantly outperforms the baseline recommenders and can smoothly and progressively influence a user's interest.

\end{enumerate}

The remaining parts of the paper are organized as follows.
We briefly review the related work 
% including \textit{Bayesian Persuasion} and \textit{Sequential Recommendation System} 
in Section \ref{sec:relatedwork}. 
In Section \ref{sec:framework}, we formulate the problem of \textit{IRS} and propose three frameworks, including two solutions adapted from existing \textit{URS} and our \textit{Influential Recommender Network}. 
In Section \ref{sec:experiment}, we first introduce the experimental setup and \textit{IRS} evaluation and then present a detailed discussion of the experimental results. 
Finally, we conclude our work and summarize the future directions in Section \ref{sec:conclusion}.

==> Influential RS/relatedwork.tex <==
\subsection{Bayesian Persuasion}
There have been decades of studies on how an entity (e.g., person, group, etc.) can be persuaded to change its action \cite{chaiken1987heuristic, kamenica2011bayesian, ajzen2012attitudes, jadbabaie2012non}. Persuasion can be defined as influencing behavior via the provision of information. \textit{Bayesian Persuasion} studies the persuasion problem in a rational (Bayesian) manner \cite{kamenica2011bayesian, bergemann2016information, kamenica2019bayesian}. The problem can be abstracted as a sender designing a signaling plan with the right amount of information disclosed so as to influence the behaviors of another receiver. Later, extensive works have applied the information design of \textit{Bayesian Persuasion} to real-world scenarios, such as social learning for online recommendation platform \cite{che2018recommender}, products advertisement \cite{arieli2019private}, and matching markets \cite{romanyuk2019cream}, etc. In this paper, we consider the persuasion problem from the perspective of \textit{RS}, which aims at changing the user to like an objective item by recommending a selected sequence of items to the user. In contrast to the existing works that model the persuasion problem as an information design and mechanism design problem requiring domain knowledge, our proposed work is data-driven where the persuasion is done by designing an influence path with proper machine learning techniques. To the best of our knowledge, we are the first to integrate \textit{RS} with persuasion behavior. 

\subsection{Sequential Recommendation System}
\label{subsec:seq_rs}
Given the natural sequential order of user-item interactions, the sequential recommender system (\textit{SRS}) tries to incorporate sequential signals into the next-item recommendation task. Due to the diversity and complexity of user-item interactions, \textit{SRS}s have to face several challenges \cite{ShoujingWang-ijcai2019}. 
(1) Learning higher-order long/short-term sequential dependencies. Compared to lower-order sequential, which are relatively simple and can be easily modeled with Markov chain or factorization machines, long/short-term sequential dependencies are much more complex and harder to capture because of their complicated multi-level cascading dependencies crossing multiple user-item interactions. Various approaches such as recurrent neural networks (\textit{RNN}) based models \cite{Wu2017RRN, hidasi2015session, bharadhwaj2018recgan}, graph-based models \cite{xiang2010temporal, wu2019session, wang2020global} have been applied to \textit{SRS}s due to their strength in modeling long/short-term interests.
(2) Handling user-item interaction sequences with flexible order and noise. \cite{tang2018personalized,Yuan2019} exploits the property of convolutional neural networks (\textit{CNN}) to model the flexible orders of user-item interactions. Attention models have been employed to emphasize relevant and important interactions in a sequence while downplaying irrelevant ones \cite{kang2018self, wang2018attentionbased, Ying2018, sun2019bert4rec}. (3) Handling user-item interaction sequences with heterogeneous relations and hierarchical structures. \cite{Tang2019, Wang2019} proposed mixture models to tackle the problem. The difference between \textit{SRS} and \textit{IRS} is, \textit{SRS} models the items' sequential dependencies for the next-item recommendation task, which belongs to the \textit{URS} category, while \textit{IRS} utilizes the sequential dependency information to generate influence paths towards the objective item.
 

==> cover_letter.tex <==
\noindent\textbf{Dear Reviewers:}
% \section*{Response Letter}

\noindent We appreciate the time and effort that you dedicated to handling our paper, providing feedback and giving us the opportunity to submit a revised paper. We are grateful for the insightful comments and have incorporated suggestions made by the reviewers. All changes are highlighted within the manuscript in red color. The removed text and minor changes (e.g. corrected spelling and grammar mistakes) have not been highlighted. We hereby provide a point-by-point response below:

\begin{itemize}%[leftmargin=0.4cm]
    \item We have clarified a few confusing points raised by the reviewers, including the use of the testing dataset (as suggested by \textbf{Reviewer #4 O1}) at the end of Section IV-A, and replaced the term ``horizon" with ``interest" (as suggested by \textbf{Reviewer #7 O1}). 
    \item Following the suggestions by \textbf{Reviewer #5 O2}, we add comments in the experimental results (Section IV-D-6) regarding the scalability and robustness of the model.
    \item \textbf{Reviewer #7 O2\&O3} suggests comparing the proposed framework to traditional methods (e.g., minimum spanning tree, search algorithm, and shortest path algorithms).
    Following this suggestion, we replace one naive baseline solution \textit{Vec2Inf} with \textit{Pf2Inf} that adapts path-finding algorithms to the influential recommendation framework. We describe the new baseline framework in Section III-B. In the experiments, we added two new baseline approaches (i.e., Dijkstra and MST) under the \textit{Pf2Inf} framework. The experimental results are presented and discussed in Section IV-D. We also extended the future work regarding the traditional methods in Section V.
\end{itemize}
%Thanks again for all the time and patience of the anonymous reviewers. 
We will also publicly release the full code and scripts on GitHub upon acceptance (suggested by \textbf{Reviewer #5 O1}). 
